Tiny Machine Learning: Progress and Futures

Tiny Machine Learning (TinyML) is a new frontier of machine learning. By squeezing deep learning models into billions of IoT devices and microcontrollers (MCUs), we expand the scope of AI applications and enable ubiquitous intelligence. However, TinyML is challenging due to hardware constraints: the tiny memory resource makes it difficult to hold deep learning models designed for cloud and mobile platforms. There is also limited compiler and inference engine support for bare-metal devices. Therefore, we need to co-design the algorithm and system stack to enable TinyML. In this review, we will first discuss the definition, challenges, and applications of TinyML. We then survey the recent progress in TinyML and deep learning on MCUs. Next, we will introduce MCUNet, showing how we can achieve ImageNet-scale AI applications on IoT devices with system-algorithm co-design. We will further extend the solution from inference to training and introduce tiny on-device training techniques. Finally, we present future directions in this area. Today's large model might be tomorrow's tiny model. The scope of TinyML should evolve and adapt over time.

==> figure_text/dlg_algorithm.tex <==
\begin{algorithm}[t]
    \caption{Deep Leakage from Gradients.}
    \label{algorithm:deep_leakage}
    \hspace*{\algorithmicindent} \textbf{Input:} 
        $F(\mathbf{x};W)$: Differentiable machine learning model;
        $W$: parameter weights; $\nabla W$: gradients calculated by training data
    \\
    \hspace*{\algorithmicindent} \textbf{Output:} private training data $\mathbf{x}, \mathbf{y}$ 
    \begin{algorithmic}[1]
    \Procedure{DLG}{$F$, $W$, $\nabla W$} % \Comment{The}
        \State $\mathbf{x'}_{1} \gets \mathcal{N}(0, 1)$ 
               , $\mathbf{y'}_{1} \gets \mathcal{N}(0, 1)$ 
        \Comment{Initialize dummy inputs and labels.}
        \For{$i \gets 1 \textrm{ to } n$}
                \State $
                    \nabla W'_i \gets 
                        \partial \ell (F(\mathbf{x'}_i, W_{t}), \mathbf{y'}_i)
                        /
                        \partial W_t
                    $ \Comment{Compute dummy gradients.} 
                \State 
                    $ \mathbb{D}_i \gets ||\nabla W'_i - \nabla W||^2 $ 
                    % \Comment{Compute distance between two gradients.}
                \State 
                    $\mathbf{x}'_{i+1} \gets \mathbf{x}'_i - \eta \nabla_{\mathbf{x}'_i} \mathbb{D}_i$
                   ,
                    $\mathbf{y}'_{i+1} \gets \mathbf{y}'_i - \eta \nabla_{\mathbf{y}'_i} \mathbb{D}_i$
                    \Comment{Update data to match gradients.}
        \EndFor
        \State \textbf{return} $\mathbf{x}'_{n+1}, \mathbf{y}'_{n+1}$
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> figure_text/dlg_defense.tex <==
\newcommand{\lgcmark}{\textcolor{green}{\cmark}}
\newcommand{\lgxmark}{\textcolor{red}{\xmark}}

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figures/fig4}
    % \caption{Caption \SH{font size should be as large as main text; reduce the space between the two rows}}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_gaussian-crop.pdf}
        \caption{Defend with different magnitude Gaussian noise.}
        \label{fig:defense:gaussian}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_laplacian-crop.pdf}
        \caption{Defend with different magnitude Laplacian noise.}
        \label{fig:defense:Laplacian}
    \end{subfigure} 
    \\ \vspace{4pt}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_fp16-crop.pdf}
        \caption{Defend with fp16 convertion.}
        \label{fig:defense:fp16}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_dgc-crop.pdf}
        \caption{Defend with gradient pruning.}
        \label{fig:defense:dgc}
    \end{subfigure} 
    \caption{The effectiveness of various defense strategies. }
    \label{fig:defense}
    \vspace{-5pt}
\end{figure}
% 
\begin{table}[t]
\setlength{\tabcolsep}{3.5pt}
\centering
\footnotesize{
\begin{tabular}[t]{c||c||c|c|c|c||c|c|c|c||c}
    & Original  & \textbf{G}-$10^{-4}$ & \textbf{G}-$10^{-3}$ & \textbf{G}-$10^{-2}$ & \textbf{G}-$10^{-1}$  & \textbf{FP}-16  \\ \hline
    Accuracy & 76.3\% & 75.6\% & 73.3\% & 45.3\% & $\le$1\% & 76.1\% \\ \hline
    Defendability & -- & \lgxmark &  \lgxmark & \lgcmark &  \lgcmark & \lgxmark \\ \hline
    % 
    &     & \textbf{L}-$10^{-4}$ & \textbf{L}-$10^{-3}$ & \textbf{L}-$10^{-2}$ & \textbf{L}-$10^{-1}$  & \textbf{Int}-8  \\ \hline
    Accuracy & -- & 75.6\% & 73.4\% & 46.2\% & $\le$1\% & 53.7\% \\ \hline
    Defendability & -- & \lgxmark &  \lgxmark & \lgcmark &  \lgcmark & \lgcmark \\
\end{tabular}
}
\caption{The trade-off between accuracy and defendability. \textbf{G}: Gaussian noise, \textbf{L}: Laplacian noise, \textbf{FP}: Floating number, \textbf{Int}: Integer quantization.
\lgcmark~means it successfully defends against DLG while \lgxmark~means fails to defend (whether the results are visually recognizable). The accuracy is evaluated on CIFAR-100.
}
\label{tab:defense_vs_accuracy}
\vspace{-10pt}
\end{table}

==> figures/defense.tex <==
\newcommand{\lgcmark}{\textcolor{green}{\cmark}}
\newcommand{\lgxmark}{\textcolor{red}{\xmark}}

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figures/fig4}
    % \caption{Caption \SH{font size should be as large as main text; reduce the space between the two rows}}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_gaussian-crop.pdf}
        \caption{Defend with different magnitude Gaussian noise.}
        \label{fig:defense:gaussian}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_laplacian-crop.pdf}
        \caption{Defend with different magnitude Laplacian noise.}
        \label{fig:defense:Laplacian}
    \end{subfigure} 
    \\ \vspace{4pt}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_fp16-crop.pdf}
        \caption{Defend with fp16 convertion.}
        \label{fig:defense:fp16}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5_dgc-crop.pdf}
        \caption{Defend with gradient pruning.}
        \label{fig:defense:dgc}
    \end{subfigure} 
    \caption{The effectiveness of various defense strategies. }
    \label{fig:defense}
    \vspace{-5pt}
\end{figure}
% 
\begin{table}[t]
\setlength{\tabcolsep}{3.5pt}
\centering
\footnotesize{
\begin{tabular}[t]{c||c||c|c|c|c||c|c|c|c||c}
    & Original  & \textbf{G}-$10^{-4}$ & \textbf{G}-$10^{-3}$ & \textbf{G}-$10^{-2}$ & \textbf{G}-$10^{-1}$  & \textbf{FP}-16  \\ \hline
    Accuracy & 76.3\% & 75.6\% & 73.3\% & 45.3\% & $\le$1\% & 76.1\% \\ \hline
    Defendability & -- & \lgxmark &  \lgxmark & \lgcmark &  \lgcmark & \lgxmark \\ \hline
    % 
    &     & \textbf{L}-$10^{-4}$ & \textbf{L}-$10^{-3}$ & \textbf{L}-$10^{-2}$ & \textbf{L}-$10^{-1}$  & \textbf{Int}-8  \\ \hline
    Accuracy & -- & 75.6\% & 73.4\% & 46.2\% & $\le$1\% & 53.7\% \\ \hline
    Defendability & -- & \lgxmark &  \lgxmark & \lgcmark &  \lgcmark & \lgcmark \\
\end{tabular}
}
\caption{The trade-off between accuracy and defendability. \textbf{G}: Gaussian noise, \textbf{L}: Laplacian noise, \textbf{FP}: Floating number, \textbf{Int}: Integer quantization.
\lgcmark~means it successfully defends against DLG while \lgxmark~means fails to defend (whether the results are visually recognizable). The accuracy is evaluated on CIFAR-100.
}
\label{tab:defense_vs_accuracy}
\vspace{-10pt}
\end{table}

==> figures/experiments/nlp.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{p{0.10\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}}
         & Example 1 & Example 2 & Example 3\\ \hline
        Initial Sentence
        & tilting fill given **less word **itude fine **nton overheard living vegas **vac **vation *f forte **dis cerambycidae ellison **don yards marne **kali
        & toni **enting asbestos cutler km nail **oof **dation **ori righteous **xie lucan **hot **ery at **tle ordered pa **eit smashing proto
        & [MASK] **ry toppled **wled major relief dive displaced **lice [CLS] us apps \_ **face **bet
    \\ \hline
        Iters = 10 
        & tilting fill given **less full solicitor other ligue shrill living vegas rider treatment carry played sculptures lifelong ellison net yards marne **kali
        & toni **enting asbestos cutter km nail undefeated **dation hole righteous **xie lucan **hot **ery at **tle ordered pa **eit smashing proto
        & [MASK] **ry toppled identified major relief gin dive displaced **lice doll us apps \_ **face space
    \\ \hline
        Iters = 20 
        & registration , volunteer applications , at student travel application open the ; week of played ; child care will be glare .
        & we welcome proposals for tutor **ials on either core machine denver softly or topics of emerging importance for machine learning .
        & one **ry toppled hold major ritual ' dive annual conference days 1924 apps novelist dude space
    \\ \hline
        Iters = 30 
        & registration , volunteer applications , and student travel application open the first week of september . child care will be available .
        & we welcome proposals for tutor **ials on either core machine learning topics or topics of emerging importance for machine learning .
        & we invite submissions for the thirty - third annual conference on neural information processing systems .
    \\ \hline
        Original Text 
        & Registration, volunteer applications, and student travel application open the first week of September. Child care will be available.
        & We welcome proposals for tutorials on either core machine learning topics or topics of emerging importance for machine learning.
        & We invite submissions for the Thirty-Third Annual Conference on Neural Information Processing Systems.
    \end{tabular}
    \caption{The progress of deep leakage on language tasks. }
    \vspace{-5pt}
    \label{tab:experiment_nlp}
\end{table}

==> figures/experiments/vision.tex <==
\newcommand\imgwidth{0.080}

\begin{figure*}[t]
    \centering
    \begin{tabular}{c c c c c | c | c}
      Iters=0 & Iters=10 & Iters=50 & Iters=100 & Iters=500 & Melis~\cite{Melis2018unintended} & Ground Truth \\
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/ground_truth.png} 
      \\ 
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/ground_truth.png} 
      \\
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/ground_truth.png}
      \\
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/ground_truth.png}
      \\
    \end{tabular}
    \caption{The visualization showing the deep leakage on images from MNIST~\cite{lecun1998mnist}, CIFAR-100~\cite{krizhevsky2009cifar}, SVHN~\cite{netzer2011svhn} and LFW~\cite{LFWTech} respectively. 
    DLG~\cite{zhu2019dlg} fully recovers the four images while previous work only succeeds on simple images with clean backgrounds.
    }
    \label{fig:experiment_vision}
    \label{fig:dlg_vision}
\end{figure*}

==> figures/experiments/vision_compare.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c c}
        \begin{minipage}[b]{0.5\linewidth}
            \includegraphics[width=\linewidth]{figures/fig3-crop.pdf}
            \captionof{figure}{Layer-$i$ means MSE between real and dummy gradients of $i^{th}$ layer.
            When the gradients' distance gets smaller, the MSE between leaked image and the original image also gets smaller.
            }
            \label{fig:vision_fig3}
        \end{minipage}
        &  
        \begin{minipage}[b]{0.45\linewidth}
        % \vspace{-20pt}
            \includegraphics[width=\linewidth]{figures/fig4_barchart-crop.pdf}
            \captionof{figure}{Compassion of the MSE of images leaked by different algorithms and the ground truth. Our method consistently outperforms previous approach by a large margin.
            }
            \label{fig:vision_fig_bar}
        \end{minipage} 
    \end{tabular}
    \vspace{-10pt}
\end{table}

==> figures/experiments/vision_multibatch.tex <==
\newcommand{\bigcell}[2]{
    \begin{tabular}{@{}#1@{}}
        #2
    \end{tabular}
}

\begin{figure}[t]
    \centering
    \small
    \begin{tabular}{c c c c c c c c c c}
      % Iters=0 & Iters=10 & Iters=50 & Iters=100 & Iters=500 & Melis~\cite{Melis2018unintended} & Ground Truth \\
        Initial     &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-0.png} 
      \\ 
        Middle Stage   &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-100.png} 
      \\
        Fully  Leaked &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-400.png} 
      \\ % \hline
        Ground  Truth &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-ground-truth.png} 
      \\
    \end{tabular}
    \caption{Results of deep leakage of batched data. Though the order may not be the same and there are more artifact pixels, DLG still produces images very close to the original ones.}
    \label{fig:experiment_vision_multi_batch}
    \vspace{-10pt}
\end{figure}

==> figures/nlp.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{p{0.10\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}}
         & Example 1 & Example 2 & Example 3\\ \hline
        Initial Sentence
        & tilting fill given **less word **itude fine **nton overheard living vegas **vac **vation *f forte **dis cerambycidae ellison **don yards marne **kali
        & toni **enting asbestos cutler km nail **oof **dation **ori righteous **xie lucan **hot **ery at **tle ordered pa **eit smashing proto
        & [MASK] **ry toppled **wled major relief dive displaced **lice [CLS] us apps \_ **face **bet
    \\ \hline
        Iters = 10 
        & tilting fill given **less full solicitor other ligue shrill living vegas rider treatment carry played sculptures lifelong ellison net yards marne **kali
        & toni **enting asbestos cutter km nail undefeated **dation hole righteous **xie lucan **hot **ery at **tle ordered pa **eit smashing proto
        & [MASK] **ry toppled identified major relief gin dive displaced **lice doll us apps \_ **face space
    \\ \hline
        Iters = 20 
        & registration , volunteer applications , at student travel application open the ; week of played ; child care will be glare .
        & we welcome proposals for tutor **ials on either core machine denver softly or topics of emerging importance for machine learning .
        & one **ry toppled hold major ritual ' dive annual conference days 1924 apps novelist dude space
    \\ \hline
        Iters = 30 
        & registration , volunteer applications , and student travel application open the first week of september . child care will be available .
        & we welcome proposals for tutor **ials on either core machine learning topics or topics of emerging importance for machine learning .
        & we invite submissions for the thirty - third annual conference on neural information processing systems .
    \\ \hline
        Original Text 
        & Registration, volunteer applications, and student travel application open the first week of September. Child care will be available.
        & We welcome proposals for tutorials on either core machine learning topics or topics of emerging importance for machine learning.
        & We invite submissions for the Thirty-Third Annual Conference on Neural Information Processing Systems.
    \end{tabular}
    \caption{The progress of deep leakage on language tasks. }
    \vspace{-5pt}
    \label{tab:experiment_nlp}
\end{table}

==> figures/vision.tex <==
% \newcommand\imgwidth{0.080}

\begin{figure}[t]
    \centering
    \begin{tabular}{c c c c c | c | c}
      Iters=0 & Iters=10 & Iters=50 & Iters=100 & Iters=500 & Melis~\cite{Melis2018unintended} & Ground Truth \\
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/mnist_0_ours/ground_truth.png} 
      \\ 
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/cifar100_25_ours/ground_truth.png} 
      \\
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/svhn_1_ours/ground_truth.png}
      \\
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0000.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0020.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0050.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0100.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/0500.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_others/unintended.png} &
        \includegraphics[width=\imgwidth\linewidth]{figures/experiments/lfw_51_ours/ground_truth.png}
      \\
    \end{tabular}
    \caption{The visualization showing the deep leakage on images from MNIST~\cite{lecun1998mnist}, CIFAR-100~\cite{krizhevsky2009cifar}, SVHN~\cite{netzer2011svhn} and LFW~\cite{LFWTech} respectively. 
    Our algorithm fully recovers the four images while previous work only succeeds on simple images with clean backgrounds.
    % More examples can be found in appendix. \zhijian{I think one visualization for the history should be enough; we can put more final results}
    }
    \label{fig:experiment_vision}
\end{figure}

==> figures/vision_compare.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c c}
        \begin{minipage}[b]{0.5\linewidth}
            \includegraphics[width=\linewidth]{figures/fig3-crop.pdf}
            \captionof{figure}{Layer-$i$ means MSE between real and dummy gradients of $i^{th}$ layer.
            When the gradients' distance gets smaller, the MSE between leaked image and the original image also gets smaller.
            }
            \label{fig:vision_fig3}
        \end{minipage}
        &  
        \begin{minipage}[b]{0.45\linewidth}
        % \vspace{-20pt}
            \includegraphics[width=\linewidth]{figures/fig4_barchart-crop.pdf}
            \captionof{figure}{Compassion of the MSE of images leaked by different algorithms and the ground truth. Our method consistently outperforms previous approach by a large margin.
            }
            \label{fig:vision_fig_bar}
        \end{minipage} 
    \end{tabular}
    \vspace{-10pt}
\end{table}

==> figures/vision_multibatch.tex <==
\newcommand{\bigcell}[2]{
    \begin{tabular}{@{}#1@{}}
        #2
    \end{tabular}
}

\begin{figure}[t]
    \centering
    \small
    \begin{tabular}{c c c c c c c c c c}
      % Iters=0 & Iters=10 & Iters=50 & Iters=100 & Iters=500 & Melis~\cite{Melis2018unintended} & Ground Truth \\
        Initial     &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-0.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-0.png} 
      \\ 
        Middle Stage   &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-100.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-100.png} 
      \\
        Fully  Leaked &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-400.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-400.png} 
      \\ % \hline
        Ground  Truth &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/0-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/1-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/2-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/3-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/4-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/5-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/6-ground-truth.png} &
        \includegraphics[width=\imgwidth\linewidth]{experiments/multi_batch/7-ground-truth.png} 
      \\
    \end{tabular}
    \caption{Results of deep leakage of batched data. Though the order may not be the same and there are more artifact pixels, DLG still produces images very close to the original ones.}
    \label{fig:experiment_vision_multi_batch}
    \vspace{-10pt}
\end{figure}

==> mcunetv1/figure_text/fig_acc_flops.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.3\textwidth]{mcunetv1/figures/acc_flops_sep.pdf}
    \caption{Distribution of Acc-log(FLOPs). TODO .}
    \label{fig:acc_flops}
\end{figure*}


==> mcunetv1/figure_text/fig_cdf.tex <==

\begin{figure*}[t]
    \centering
     \includegraphics[width=1.0\textwidth]{mcunetv1/figures/cdf.pdf}
     % \vspace{-15pt}
    \caption{TinyNAS selects the best search space by analyzing the FLOPs CDF of different search spaces.
    % \SH{prerequisite: has to satisfy hardware constraints}
    Each curve represents a design space.
    % The design space with a higher average FLOPs is more likely to produce high performance models 
    Our insight is that the design space that is more likely to produce \textit{high FLOPs} models under the memory constraint gives higher model capacity, thus more likely to achieve high accuracy.
    For the solid \textcolor{red}{\textbf{red}}  space, the top 20\% of the models have $>$50.3M FLOPs, while for the solid  \textbf{black}  space, the top 20\% of the models only have $>$32.3M FLOPs. Using the solid \textcolor{red}{\textbf{red}}  space for neural architecture search achieves 78.7\% final accuracy, which is 4.5\% higher compared to using the {\textbf{black}}  space.
    The legend is in format: \texttt{w\{width\}-r\{resolution\}|\{mean FLOPs\}}. 
    % Using a width multiplier of 0.5 and an input resolution of 144 achieves the best model distribution on ImageNet-100 with 320kB SRAM and 1MB Flash.
    }
    \label{fig:cdf}
    % \vspace{-15pt}
\end{figure*}

==> mcunetv1/figure_text/fig_compare_resnet18.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/compare_resnet18.pdf}
%     \caption{MCUNet achieves slightly better accuracy than ResNet-18 (70.2\% \vs 69.8\%) while using \textbf{7.8$\times$} less SRAM memory  and \textbf{26.2$\times$} less Flash.
%     % \SH{reviewers would ask how many bits are there for the ResNet18? if not the focus we can delete 4bit next to the MCUNet.}
%     }
%     \label{fig:compare_resnet18}
% \end{figure*}


==> mcunetv1/figure_text/fig_gcommands_curve.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/gcommands_curve.pdf}
%     \caption{Speech Commands results. TODO .}
%     \label{fig:gcommands_curve}
% \end{figure*}


==> mcunetv1/figure_text/fig_grid_config.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{mcunetv1/figures/grid_config_width_circle.pdf}
         \caption{Best width setting.}
         \label{fig:grid_config_width}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{mcunetv1/figures/grid_config_resolution_circle.pdf}
         \caption{Best resolution setting.}
         \label{fig:grid_config_res}
     \end{subfigure}
     % \vspace{-5pt}
        \caption{Best search space configurations under different SRAM and Flash constraints.}
        \label{fig:grid_config}
        % \vspace{-15pt}
\end{figure*}

==> mcunetv1/figure_text/fig_memory_ablation.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{mcunetv1/figures/memory_ablation_bars.pdf}
    % \vspace{-15pt}
    \caption{TinyEngine reduces peak memory by eliminating memory usage of interpreters and updating activations of depth-wise convolutions in-place, enlarging design space for TinyNAS under a given memory constraint.}
    % \vspace{-15pt}
    \label{fig:memory_ablation_bars}
\end{figure*}


==> mcunetv1/figure_text/fig_speedup.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{mcunetv1/figures/speedup.pdf}
    \caption{TinyEngine outperforms existing inference frameworks while reducing peak memory for running typical networks. The x axis labels are in format: \texttt{\{model\}-r\{resolution\}}. \textbf{Up}: By reducing memory usage, TinyEngine can run higher resolutions within the memory constraint for a given model. \textbf{Down}: TinyEngine outperforms existing frameworks for each model at various resolutions. Note that if the required memory of a setting exceeds the memory constraint, its bar is shown as OOM. }
    \label{fig:speedup}
\end{figure*}

==> mcunetv1/figure_text/fig_speedup_ablation.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{mcunetv1/figures/speedup_breakdown.pdf}
    % \includegraphics[width=0.8\textwidth]{figures/speedup_ablation.pdf}
    % \vspace{-15pt}
    \caption{TinyEngine outperforms existing libraries by eliminating runtime overheads and specializing each optimization technique. This effectively enlarges design space for TinyNAS under a given latency constraint.}
    \label{fig:speedup_ablation}
    % \vspace{-10pt}
\end{figure*}


==> mcunetv1/figure_text/fig_vww_curve.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/vww_curve.pdf}
%     \caption{VWW Results. TODO .}
%     \label{fig:vww_curve}
% \end{figure*}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/vww_curve.pdf}
%     \includegraphics[width=0.95\textwidth]{figures/gcommands_curve.pdf}
%     \caption{Top: VWW; Bottom: Speech Commands results}
%     \label{fig:vww_curve}
%     \label{fig:gcommands_curve}
% \end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{mcunetv1/figures/vww_gsc_curves_ipdw.pdf}
    \caption{Accuracy \vs latency/SRAM memory trade-off on VWW (\textbf{top}) and Speech Commands (\textbf{down}) dataset. MCUNet achieves better accuracy while being 2.4-3.4$\times$ faster at 3.7-4.1$\times$ smaller peak SRAM.}
    \label{fig:vww_curve}
    \label{fig:gcommands_curve}
    % \vspace{-10pt}
\end{figure*}

==> mcunetv1/figure_text/tab_4bit.tex <==
\begin{figure*}[t]
\begin{minipage}[b]{\textwidth}
\setlength{\tabcolsep}{4pt}
\captionof{table}{MCUNet can handle diverse hardware resource on different MCUs. It outperforms~\cite{rusci2019memory} without using advanced mixed-bit quantization (8/4/2-bit) policy under different resource constraints, achieving a record ImageNet accuracy (>70\%) on microcontrollers.}
\vspace{-5pt}
\label{tab:4bit}
\begin{center}
\small{
   \begin{tabular}{lccccc}
\toprule
% \textbf{Constraints} 
& Quantization &  \shortstack{STM32F412\\(256kB, 1MB)}  & \shortstack{STM32F746\\(320kB, 1MB)}   & \shortstack{STM32F765\\(512kB, 1MB)} &   \shortstack{STM32H743\\(512kB, 2MB)} \\  
\midrule
\textbf{Rusci \etal}~\cite{rusci2019memory} & Mixed  & 60.2\% & - & 62.9\% & 68.0\%  \\ 
% 1.5s, -, 2.0s, 3.9s
% \midrule
\textbf{MCUNet} & 4-bit  &  \textbf{62.0\%} & \textbf{63.5\%} & \textbf{65.9\%} &  \textbf{70.7\%} \\ 
% \textbf{MCUNet} & 8-bit  &  -  & 60.1\%  & - & - \\  % / 1.1s
%  / 1.1s, 1.6s, 3.0s, 3.5s
\bottomrule
 \end{tabular}
}
\end{center}
\end{minipage}
~~~~~~~
\begin{minipage}[b]{\textwidth}
\centering
    \centering
    \vspace{15pt}
    \includegraphics[width=\textwidth]{mcunetv1/figures/compare_resnet18_mbv2_ipdw.pdf}
    % \caption{MCUNet reduces the the Flash usage by \textbf{26.2$\times$} and SRAM memory by \textbf{7.8$\times$} than ResNet18, while achieving better accuracy (70.2\% \vs 69.8\% ImageNet top-1).
     \caption{MCUNet reduces the the SRAM memory by \textbf{3.5$\times$} and Flash usage by \textbf{5.7$\times$} compared to MobileNetV2 and ResNet-18 (8-bit), while achieving better accuracy (70.7\% \vs 69.8\% ImageNet top-1).
    }
    \label{fig:compare_resnet18}
\end{minipage}
\vspace{-10pt}
\end{figure*}


==> mcunetv1/figure_text/tab_codesign.tex <==
% % \renewcommand \arraystretch{0.9}
% \begin{table}[t]
% % \setlength{\tabcolsep}{4pt}
% % \vspace{-20pt}
% \caption{System-algorithm co-design (TinyEngine+TinyNAS) achieves the highest ImageNet accuracy of models runnable on a microcontroller (320kB SRAM, 1MB Flash).}
% \label{tab:codesign}
% \begin{center}
% \small{
%   \begin{tabular}{l|ccc}
% \toprule
% % \textbf{Constraints} 
% \backslashbox{Library}{Model} & S-MbV2 &  S-Proxyless  & TinyNAS   \\  
% \midrule
% CMSIS-NN~\cite{lai2018cmsis} & 35.2\%  & 49.5\% & 55.5\% \\ 
% TinyEngine & 43.8\%  &  54.4\% & \textbf{60.1\%}  \\
% \bottomrule
%  \end{tabular}
% }
% \end{center}
% \end{table}



\begin{figure*}[t]
\begin{minipage}[b]{0.5\textwidth}
\renewcommand \arraystretch{1.2}
\centering
\setlength{\tabcolsep}{2pt}
\captionof{table}{System-algorithm co-design (TinyEngine + TinyNAS) achieves the highest ImageNet accuracy of models runnable on a microcontroller.
% (320kB SRAM, 1MB Flash).
}
\label{tab:codesign}
\small{
   \begin{tabular}{lccc}
\toprule
% \textbf{Constraints} 
Library\textbackslash Model & S-MbV2 &  S-Proxyless  & TinyNAS   \\  
\midrule
CMSIS-NN~\cite{lai2018cmsis} & 35.2\%  & 49.5\% & 55.5\% \\ 
TinyEngine & 47.4\%  &  56.4\% & \textbf{61.8\%}  \\
\bottomrule
 \end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\textwidth}
\centering
\setlength{\tabcolsep}{2pt}
\captionof{table}{MCUNet outperforms the baselines at various latency requirements. Both TinyEngine and TinyNAS bring significant improvement on ImageNet.}
\label{tab:latency_imagenet}
\small{
   \begin{tabular}{lccc}
\toprule
% \textbf{Constraints} 
 \textbf{Latency Constraint} & \textbf{N/A} &  \textbf{5FPS}  & \textbf{10FPS}  \\  
\midrule
S-MbV2+CMSIS & 39.7\% & 39.7\% & 28.7\% \\ 
S-MbV2+TinyEngine & 47.4\% & 41.6\% & 34.1\% \\\midrule
MCUNet & \textbf{61.8\%} & \textbf{49.9\%} & \textbf{40.5\%} \\
\bottomrule
 \end{tabular}
}
\end{minipage}
\vspace{-5pt}
\end{figure*}




==> mcunetv1/figure_text/tab_detection.tex <==
% \setlength{\columnsep}{3pt}%
% \begin{wrapfigure}{r}{0.25\textwidth}
%     \setlength{\tabcolsep}{3pt}
%     \vspace{-10pt}
%     \captionof{table}{Detection results.}
%     \label{tab:detection}
%     \small{
%      \begin{tabular}{l|c}
%     \toprule
%       & mAP  \\  
%     \midrule
%     MbV2+CMSIS & 31.6\%\\ 
%     MCUNet &  \textbf{51.4\%}\\
%     \bottomrule
%      \end{tabular}
%      }
%      \vspace{-15pt}
% \end{wrapfigure}


\setlength{\columnsep}{3pt}%
\begin{table}[t]
    \setlength{\tabcolsep}{3pt}
    \vspace{-5pt}
    \caption{MCUNet improves the detection mAP by 20\% on Pascal VOC under 512kB SRAM constraint. With MCUNet, we are able to fit a model with much larger capacity and computation FLOPs at a smaller peak memory. MobileNet-v2 + CMSIS-NN is bounded by the memory consumption: it can only fit a model with 34M FLOPs even when the peak memory slightly exceeds the budget, leading to inferior detection performance.}
    \vspace{5pt}
    \label{tab:detection}
    \centering
    \small{
     \begin{tabular}{l|cccc|c}
    \toprule
      & resolution & FLOPs & \#Param & peak SRAM & mAP  \\  
    \midrule
    MbV2+CMSIS & 128 & 34M & 0.87M & \textcolor{gray}{519kB (OOM)} & 31.6\%\\ 
    MCUNet & 224 & 168M & 1.20M & 466kB  &  \textbf{51.4\%}\\
    \bottomrule
     \end{tabular}
     }
     \vspace{-15pt}
\end{table}

==> mcunetv1/figure_text/tab_fig_spaces.tex <==
\begin{figure*}[t]
\begin{minipage}[b]{0.6\textwidth}
\centering
\setlength{\tabcolsep}{3.5pt}
\small{
\begin{tabular}{lcccc}
\toprule
 & \textcolor{gray}{R-18@224}  & Rand Space & Huge Space & Our Space \\  
\midrule
    \textbf{Acc.} & \textcolor{gray}{80.3\%} & 74.7$\pm$1.9\% & 77.0\%   & \textbf{78.7\%} \\
\bottomrule
 \end{tabular}
 }
 \captionof{table}{Our search space achieves the best accuracy, closer to ResNet-18@224 resolution (\textcolor{gray}{OOM}). Randomly sampled and a huge space (contain many configs) leads to worse accuracy.}
 \label{tab:acc_vs_space}
\end{minipage}
\hfill
\begin{minipage}[b]{0.37\textwidth}
\centering
\includegraphics[width=\textwidth]{mcunetv1/figures/acc_vs_auc.pdf}
\caption{Search space with higher mean FLOPs leads to higher final accuracy.}
 \label{fig:acc_vs_auc}
\end{minipage}
\vspace{-5pt}
\end{figure*}


==> mcunetv1/figure_text/tab_imagenet_latency.tex <==
% \renewcommand \arraystretch{0.9}
\begin{table}[t]
% \setlength{\tabcolsep}{4pt}
% \vspace{-20pt}
\caption{MCUNet outperforms the baselines at various latency requirements.}
\label{tab:codesign}
\begin{center}
\small{
   \begin{tabular}{lccc}
\toprule
% \textbf{Constraints} 
 \textbf{Latency} & \textbf{N/A} &  \textbf{5FPS}  & \textbf{10FPS}  \\  
\midrule
MbV2+CMSIS &  \\ 
MbV2+TinyEngine & 43.8\% & 41.6\% & 34.1\% \\\midrule
MCUNet & \textbf{60.1\%} & \textbf{49.9\%} & \textbf{40.5\%} \\
\bottomrule
 \end{tabular}
}
\end{center}
\end{table}





==> mcunetv1/figure_text/tab_wake_words.tex <==
\renewcommand \arraystretch{1.1}
\begin{table}[t]
\caption{MCUNet consistently outperforms baseline models on various datasets and resource constraints. All the models are profiled using TinyEngine. \ji{the improvement seems small on VWW and GCommands. Consider remove them and plot something like Acc.\vs Memory.}}
\label{tab:wake_words}
\small
\begin{center}
\begin{tabular}{ccccccc}
\toprule
\textbf{Dataset} & \textcolor{gray}{\textbf{ResNet-18@224}} & \textbf{Constraints} &  \textbf{S-MbV2} &  \textbf{S-Proxyless} &  \textbf{Lin et al.} & \textbf{MCUNet}  \\ 
\toprule
%%% ImageNet
% MCU1
\multirow{2}{*}{ImageNet} & \multirow{2}{*}{\textcolor{gray}{69.8\%}}  & (320kB, 1MB) 
& 43.8\%  % mbv2_imagenet_r0.3_r128.tflite
& 54.4\%  % proxylessmobile_imagenet_r0.2_r176.tflite
& - 
& 60.2\%  % model-IN-evolve_1000_ram320_flash1024.tflite
\\ \cmidrule(l){3-7}
% MCU2
& & (512kB, 2MB) 
& 58.6\%  % mbv2_imagenet_w0.5_r160.tflite
&  
& -  & 65.1\% \textcolor{red}{I8}   \\  
 \midrule
%%% VWW
\multirow{2}{*}{VWW} &  \multirow{2}{*}{\textcolor{gray}{92.9\%}}  &  (320kB, 1MB) 
& 89.8\%   % mbv2_vww_w0.4_r128.tflite
& 90.4\%  % pmobile_vww_w0.4_r144.tflite
&  90.7\% \textcolor{red}{I8}
& 92.0\%% vww_ram320_flash1024.tflite
\\  \cmidrule(l){3-7}
 & & (512kB, 2MB) 
 &    
 &  
 & 92.0\% \textcolor{red}{I8}
 &  92.4\% \textcolor{red}{I8}   \\  
\midrule
%%% GCommands
\multirow{2}{*}{\shortstack{Speech\\Commands}}  & \multirow{2}{*}{\textcolor{gray}{96.7\%}} & (320kB, 1MB) 
&  94.2\%  \textcolor{red}{I8}
&  94.4\%  \textcolor{red}{I8}
&  -
& 96.4\%  \textcolor{red}{I8}
\\  \cmidrule(l){3-7}
&  & (512kB, 2MB) 
&    
&  
&  
& 96.8\%  \textcolor{red}{I8} \\  
\bottomrule
\end{tabular}
\end{center}
% \vspace{-15pt}
\end{table}

==> mcunetv1/main.tex <==

\input{mcunetv1/text/0_abstract}
\input{mcunetv1/text/1_introduction}
\input{mcunetv1/text/2_related_work}
\input{mcunetv1/text/3_approach}
\input{mcunetv1/text/4_experiments}
\input{mcunetv1/text/5_conclusion}



==> mcunetv1/text/0_abstract.tex <==

\begin{abstract}
Machine learning on tiny IoT devices based on microcontroller units (MCU) is appealing but challenging:
the memory of microcontrollers
is 2-3 orders of magnitude smaller even than mobile phones.
We propose MCUNet, a framework that jointly designs the efficient neural architecture (TinyNAS) and the lightweight inference engine (TinyEngine), enabling ImageNet-scale inference on microcontrollers. 
TinyNAS adopts a two-stage neural architecture search approach that first optimizes the search space to fit the resource constraints,
% according to the target platform, which brings higher probability to find a high-accuracy model that fits TinyEngine, 
then specializes the network architecture in the optimized search space.
TinyNAS can automatically handle diverse constraints (\textit{i.e.} device, latency, energy, memory) under low search costs.
TinyNAS is co-designed with TinyEngine, a memory-efficient inference library to expand the search space and fit a larger model.
TinyEngine adapts the memory scheduling according to the \textit{overall} network topology rather than \textit{layer-wise} optimization, 
reducing the memory usage by $3.4\times$, and accelerating the inference by 1.7-3.3$\times$ compared to TF-Lite Micro~\cite{abadi2016tensorflow} and CMSIS-NN~\cite{lai2018cmsis}.
MCUNet is the first to achieves $>$70\% ImageNet top1 accuracy on an off-the-shelf commercial microcontroller, using 3.5$\times$ less SRAM and 5.7$\times$ less Flash compared to quantized MobileNetV2 and ResNet-18. 
% with only 1MB flash and 320KB SRAM. 
On visual\&audio wake words tasks, MCUNet 
% achieves 10 FPS, 13$\times$ faster than previous work at the same level of accuracy.
achieves state-of-the-art accuracy and runs 2.4-3.4$\times$ faster than MobileNetV2 and ProxylessNAS-based solutions with 3.7-4.1$\times$ smaller peak SRAM.
% For interactive applications, our solution achieves 10 FPS, which is 13$\times$ faster than previous work at the same level of accuracy.
% Our tiny models are energy efficient, 
% The energy consumption is so low that it can run on a button battery for 6 months.
% \ji{to check}
% To the best of our knowledge, we are the first to achieve AlexNet level accuracy ($>57.2\%$ top-1) on ImageNet running on an off-the-shelf commercial microcontroller. The model is xxx smaller, xxx less computation. The compiler is xxx faster. Overall it is xxx faster. The search cost is xxx lower. (show some large and impressive numbers here).
Our study suggests that the era of always-on tiny machine learning on IoT devices has arrived.
% We provide a demo video at: \ji{TODO}.
% \gc{abstract seems too long for me.}
% A demo video is \href{https://youtu.be/YvioBgtec4U}{here}.
% Code and models can be found here: \url{https://tinyml.mit.edu}.
\end{abstract}






==> mcunetv1/text/1_introduction.tex <==
\section{Introduction}

% IoT devices based on microcontroller units (MCU) have been deployed everywhere, enabling numerous applications including smart factory, precision agriculture, automated retail, personalized healthcare, \etc.
% Due to the low cost (average price of 60 cents per unit) and low energy consumption, microcontrollers are embracing a giant market. 
% There are 250 billions of microcontrollers in the world today,
% % powering almost all of the embedded devices, 
% and the number is still increasing at a historical rate. 

The number of IoT devices based on always-on microcontrollers is increasing rapidly at a historical rate, reaching 250B~\cite{venturebeat_tinyml}, enabling numerous applications including smart manufacturing, personalized healthcare, precision agriculture, automated retail, \etc.
These low-cost, low-energy microcontrollers give rise to a brand new opportunity of tiny machine learning (TinyML).
% \gc{The next sentence does not transit smoothly. Maybe first talk about the resource constraint on microcontrollers, and then show pity that we can not run deep model without new technique.} 
By running deep learning models on these tiny devices, we can directly perform data analytics near the sensor, thus dramatically expand the scope of AI applications.
% \ji{should we mention low cost and low energy consumption?} 
% \ji{From CMSIS-NN: Deep Neural Networks are becoming increasingly popular in always-on IoT edge devices performing data analytics right at the source, reducing latency as well as energy consumption for data communication}

However, microcontrollers have a very limited resource budget, especially memory (SRAM) and storage (Flash). The on-chip memory is 3 orders of magnitude smaller than mobile devices, and 5-6 orders of magnitude smaller than cloud GPUs, making deep learning deployment extremely difficult.
As shown in Table~\ref{tab:hardware_stats}, a state-of-the-art ARM Cortex-M7 MCU only has 320kB SRAM and 1MB Flash storage, which is impossible to run off-the-shelf deep learning models: ResNet-50~\cite{he2016deep} exceeds the storage limit by $100\times$, MobileNetV2~\cite{sandler2018mobilenetv2} exceeds the peak memory limit by $22\times$. Even the int8 quantized version of MobileNetV2 still exceeds the memory limit by $5.3\times$\footnote{Not including the runtime buffer overhead (\eg, Im2Col buffer); the actual memory consumption is larger.}, showing a big gap between the desired and available hardware capacity.



\input{mcunetv1/figure_text/fig_hardware_stats}


Different from the cloud and mobile devices, microcontrollers are bare-metal devices that do not have an operating system. 
Therefore, we need to jointly design the deep learning model and the inference library to efficiently manage the tiny resources and fit the tight memory\&storage budget. 
Existing efficient network design~\cite{howard2017mobilenets, sandler2018mobilenetv2, zhang2018shufflenet} and neural architecture search methods~\cite{tan2019mnasnet, cai2019proxylessnas, wu2019fbnet, cai2020once} focus on GPU or smartphones, where both memory and storage are abundant. Therefore, they only optimize to reduce FLOPs or latency, and the resulting models cannot fit microcontrollers. There is limited literature~\cite{fedorov2019sparse, liberis2019neural, rusci2019memory, lawrence2019iotnet} that studies machine learning  
on microcontrollers. However, due to the lack of system-algorithm co-design, they either study tiny-scale datasets (\eg, CIFAR or sub-CIFAR level), which are far from real-life use case, or use weak neural networks that cannot achieve decent performance.
% merely outperform non-deep algorithms like SVM.


In this paper, we propose MCUNet, a system-model co-design framework that enables ImageNet-scale deep learning on off-the-shelf microcontrollers. To handle the scarce on-chip memory on microcontrollers, we jointly optimize the deep learning model design (TinyNAS) and the inference library (TinyEngine) to reduce the memory usage. 
TinyNAS is a two-stage neural architecture search (NAS) method that can handle the tiny and diverse memory constraints on various microcontrollers. The performance of NAS highly depends on the search space~\cite{radosavovic2020designing}, yet there is little literature on the search space design heuristics at the tiny scale. TinyNAS addresses the problem by first optimizing the search space automatically to fit the tiny resource constraints, then performing neural architecture search in the optimized space. Specifically, TinyNAS generates different search spaces by scaling the input resolution and the model width, then collects the computation FLOPs distribution of satisfying networks within the search space to evaluate its priority. TinyNAS relies on the insight that \emph{a search space that can accommodate higher FLOPs under memory constraint can produce better model}. Experiments show that the optimized space leads to better accuracy of the NAS searched model.
% Besides the inference framework, we need specialized neural network architecture for microcontrollers to fit memory constraints.
% However, the accuracy of the searched model is largely affected by the quality of the search space~\cite{radosavovic2020designing}. 
% Traditionally, people design the search space according to the heuristics from manual design for GPUs and mobile phones. 
% However, non of these work can fit a MCU.
% In the microcontroller scenario with extremely tight on-device resource constraints, there is few existing deep networks as a reference, making search space design tough. 
% Also, the resource constraints are different from device to device, therefore a principled design methodology is required to fit the tight and diverse constraints. 
% To address it, we propose a \emph{two-step neural architecture search} method that firstly optimizes the search space under a certain resource constraints and then searches a good model inside the space. Specifically, we took a statistical approach by randomly sampling sub-networks from each search space to evaluate the overall statistics distribution. \SH{a bit vague. what statistics?} As our system optimizes the inference memory allocation according to the deep network structure, we put the inference system inside the loop to jointly optimize the neural network architecture.
% Experiments show that such design method outperforms human heuristics and random search space by a margin (Section~\textbf{TODO}).
To handle the extremely tight resource constraints on microcontrollers, we also need a memory-efficient inference library to eliminate the unnecessary memory overhead, so that we can expand the search space to fit larger model capacity with higher accuracy. TinyNAS is co-designed with TinyEngine to lift the ceiling for hosting deep learning models. TinyEngine improves over the existing inference library with code generator-based compilation method to eliminate memory overhead
% , which reduces the memory usage by $2.7\times$ and improves the inference speed by 22\%
. It also supports model-adaptive memory scheduling: instead of \textit{layer-wise} optimization, TinyEngine optimizes the memory scheduling according to the \textit{overall} network topology to get a better strategy. 
% Finally, it optimizes computation kernels in various aspects, accelerates the inference of models, and allows for a larger model capacity at the same latency constraints. \ji{remove this sentense and refine}
Finally, it performs \textit{specialized} computation kernel optimization (\eg, loop tiling, loop unrolling, op fusion, \etc) for different layers, which further accelerates the inference.
% , and allows for a larger model capacity at the same latency constraints. 

% We first propose a memory-efficient model adaptive inference library TinyEngine to host deep learning models.
% Existing inference library (TensorFlow Lite Micro, CMSIS-NN~\cite{lai2018cmsis}, MicroTVM~\cite{chen2018tvm}, etc.) is not well optimized for the scarce memory: the deployed model is first interpreted by the runtime, which will consume a large part of the SRAM and Flash (sometimes up to $65\%$ of the total used memory). The wasted memory significantly lowers the memory ceiling for running deep learning models.  To address this, we propose an efficient code generation process to eliminate the memory space required by the existing runtime. 
% Besides, we propose an advanced memory buffer allocation technique to maximize the buffer reuse by finding the optimal memory scheduling according to the overall network architecture but not single layer. \SH{by using software-managed buffer rather than hardware-managed cache?}
% We also designed specialized vectorization technique to improve inference speed. The system-level decisions are co-designed with the network architecture.
% when a hardware accelerator like DSP is available.


MCUNet dramatically pushes the limit of deep network performance on microcontrollers. TinyEngine reduces the peak memory usage by 3.4$\times$ and accelerates the inference by 1.7-3.3$\times$ compared to TF-Lite and CMSIS-NN, allowing us to run a larger model. 
% , Flash consumption \WM{maybe remove flash consumption? we don't report the improvement on storage.} and the inference latency of deep learning models. When benchmarked on STM32F746 board with Cortex-M7 core, our framework reduces the peak SRAM usage by $2.7\times$ compared to TF-Lite and CMSIS-NN, allowing us to run a larger model. \ji{maybe add tvm here later}. 
With system-algorithm co-design, MCUNet (TinyNAS+TinyEngine) achieves a record ImageNet top-1 accuracy of 70.7\% on an off-the-shelf commercial microcontroller.
% , using 7.8$\times$ smaller peak SRAM and 26.2$\times$ smaller Flash compared to the widely used ResNets.
On visual\&audio wake words tasks, MCUNet achieves state-of-the-art accuracy and runs 2.4-3.4$\times$ faster than existing solutions at 3.7-4.1$\times$ smaller peak SRAM.
% with 20-100$\times$ less memory. 
% For interactive applications, MCUNet achieves 91\% accuracy on Speech Commands dataset at 10 FPS, which is 13$\times$ faster than previous work.
For interactive applications, our solution achieves 10 FPS with 91\% top-1 accuracy on Speech Commands dataset.  Our study suggests that the era of tiny machine learning on IoT devices has arrived.


% Our framework also accelerates the inference by $3.3\times$ compared to TF-Lite and $1.7\times$ compared to CMSIS-NN. Remarkably, combined with our jointly optimized deep learning models, the principled co-design methodology achieves $60.2\%$ top-1 accuracy on ImageNet~\cite{deng2009imagenet}. To the best of our knowledge, we are the first one to achieve AlexNet-level ImageNet accuracy (plus a significant advantage) on an off-the-shelf commercial microcontrollers. 
% We also design models for latency and energy constrained models. \ji{TODO: add results}. We are able to run the network powered by a button battery for xxx month and achieve xx accuracy on VWW/GCommands.


==> mcunetv1/text/2_related_work.tex <==
\section{Background}

% \subsection{Microcontroller Basics}


% \ji{I think we need a paragraph to tell the readers how the deep learning network is inferenced on MCUs, e.g., instruction and static data is in Flash and there is no intermediate memory hierrachies. So that people can know how our optimization works.

% A good example here: https://arxiv.org/pdf/1910.05110.pdf


% % Maybe we should also say this: 
% % A backing storage, e.g. an SD-card, typically has a high capacity but is slow and power-costly to access ($\approx 100\times$ more energy required to read a value outside of on-chip memory~\cite{horowitz20141}).

% }
Microcontrollers have tight memory: for example, only 320kB SRAM and 1MB Flash for a popular ARM Cortex-M7 MCU STM32F746.
% A microcontroller unit usually consists of a low-frequency processing core and on-chip memory (read-write SRAM and read-only Flash memory). 
% \SH{doesn't add much to the paper; the only useful info is: MCU has small memory}
% In this paper, we study a widely used commercial microcontroller STM32F746NG with an Arm Cortex-M7 core, 320kB SRAM and 1MB Flash. 
% during deep network execution, including the input and output activation of the current layer, the buffer to store partial weights, the buffers for optimization (\eg, Im2col buffer), \etc. Flash is used to host the weight and architecture of the deep learning models, the program code (instructions, constant variables), and the framework interpreter (e.g., TF-Lite interpreter). 
% Different from the mobile or cloud platform, there is no other intermediate memory hierarchy. 
% Some microcontrollers support external memory like SD card. However,
% accessing the external memory is slow and consumes $100\times$ more energy compared to on-chip memory~\cite{horowitz20141}, which is prohibitive under low-power setting. 
Therefore, we have to carefully design the inference 
library and the deep learning models to fit the tight memory constraints. In deep learning scenarios, SRAM  constrains the activation size (read\&write); Flash  constrains the model size (read-only). 
% \SH{I removed a lot from this paragraph. the removed sentences doesn't add to the contribution. you're not writing a thesis: no need to cover everything, only write useful/novel key points. please use this principle to cut other paragraphs, otherwise we will run out of space.}


\myparagraph{Deep Learning Inference on Microcontrollers.}

Deep learning inference on microcontrollers is a fast-growing area. Existing frameworks such as TensorFlow Lite Micro~\cite{abadi2016tensorflow}, CMSIS-NN~\cite{lai2018cmsis}, CMix-NN~\cite{capotondi2020cmix}, and MicroTVM~\cite{chen2018tvm}
% TensorFlow Lite~\cite{abadi2016tensorflow} is among the first deep learning framework to support bare-metal microcontrollers. CMSIS-NN~\cite{lai2018cmsis} implements optimized kernels to improve the inference speed and energy efficiency. CMix-NN~\cite{capotondi2020cmix} supports mixed precision on MCU to reduce memory footprint.
% Recently, TVM~\cite{chen2018tvm} and AutoTVM~\cite{chen2018learning} also supports microcontrollers (named as $\mu$TVM/microTVM). 
% \SH{I cut a lot. no need to write a full sentence for each}
have several limitations: 1. Most frameworks rely on an interpreter to interpret the network graph at runtime, which will consume a lot of SRAM and Flash (up to $65\%$ of peak memory) and increase latency by 22\%. 2. The optimization is performed at layer-level, which fails to utilize the overall network architecture information to further reduce memory usage.


\myparagraph{Efficient Neural Network Design.}

Network efficiency is very important for the overall performance of the deep learning system. One way is to compress off-the-shelf networks by pruning~\cite{han2015learning, he2017channel, lin2017runtime, liu2017learning, he2018amc, liu2019metapruning} and quantization~\cite{han2016deep, zhu2016trained, rastegari2016xnor, zhou2016dorefa, courbariaux2016binarynet, choi2018pact, wang2019haq, langroudi2021tent} to remove redundancy and reduce complexity. Tensor decomposition~\cite{lebedev2014speeding,gong2014compressing,kim2015compression} also serves as an effective compression method. Another way is to directly design an efficient and mobile-friendly network~\cite{howard2017mobilenets, sandler2018mobilenetv2, ma2018shufflenet,zhang2018shufflenet, ma2018shufflenet}. Recently,   neural architecture search (NAS)~\cite{zoph2017neural, zoph2018learning, liu2019darts, cai2019proxylessnas, tan2019mnasnet, wu2019fbnet} dominates efficient network design. 
% based methods dominate efficient deep learning network design.

The performance of NAS highly depends on the quality of the search space~\cite{radosavovic2020designing}. Traditionally, people follow manual design heuristics for NAS search space design. For example, the widely used mobile-setting search space~\cite{tan2019mnasnet, cai2019proxylessnas, wu2019fbnet} originates from MobileNetV2~\cite{sandler2018mobilenetv2}: they both use 224 input resolution and a similar base channel number configurations, while searching for kernel sizes, block depths, and expansion ratios.
However, there lack standard model designs for microcontrollers with limited memory, so as the search space design.
% But there is no off-the-shelf network that successfully runs on memory-constrained microcontroller. Therefore, we cannot borrow form the existing effort. We need to develop techniques to automatically find a good search space for microcontroller deployment.
% Neural architecture search (NAS) dominates specialized model design under resource-constrained settings~\cite{cai2019proxylessnas, tan2019mnasnet, wu2019fbnet}.
% % Search space design is one of the key to success.
% The final accuracy highly depends on the search space design~\cite{radosavovic2020designing}. 
% Traditionally, people follow the manual model design heuristics for search space design. For example, the widely used mobile-setting search space~\cite{tan2019mnasnet, cai2019proxylessnas, wu2019fbnet, cai2020once} originates from MobileNetV2~\cite{sandler2018mobilenetv2}: they both use 224 input resolution and a similar base channel number configurations, while searching for kernel sizes, block depths, and expansion ratios. However, there lacks standard model design for microcontrollers with limited memory, so as search space design.
% making the NAS search space design difficult. 
One possible way is to manually tweak the search space for each microcontroller. But manual tuning through trials and errors is labor-intensive, making it prohibitive for a large number of deployment constraints (\eg, STM32F746 has 320kB SRAM/1MB Flash, STM32H743 has 512kB SRAM/2MB Flash, latency requirement 5FPS/10FPS). 
Therefore, we need a way to automatically optimize the search space for tiny and diverse deployment scenarios.


==> mcunetv1/text/3_approach.tex <==
\section{MCUNet: System-Algorithm Co-Design}


\input{mcunetv1/figure_text/fig_overview}

We propose MCUNet, a system-algorithm co-design framework that jointly optimizes the NN architecture (TinyNAS) and the inference scheduling (TinyEngine) in a same loop (Figure~\ref{fig:overview}). Compared to traditional methods that either (a) optimizes the neural network using neural architecture search based on a given deep learning library (\eg, TensorFlow, PyTorch)~\cite{tan2019mnasnet, cai2019proxylessnas, wu2019fbnet}, or (b) tunes the library to maximize the inference speed for a given network~\cite{chen2018tvm, chen2018learning}, MCUNet can better utilize the resources by system-algorithm co-design.
% to achieve higher accuracy on tiny hardware.

% As shown in Figure~\ref{fig:overview}, our framework consists of two parts: 1. TinyEngine: a memory-efficient \& model adaptive inference library to generate optimal inference scheduling for a given model. 2. TinyNAS: tiny NN architecture specialization to fit the resource constraints.

\subsection{TinyNAS: Two-Stage NAS for Tiny Memory Constraints}

% \ji{TODO: rewrite to echo with ``Tiny'' keyword}

TinyNAS is a two-stage neural architecture search method that first optimizes the search space to fit the tiny and diverse resource constraints, and then performs neural architecture search within the optimized space. With an optimized space, it significantly improves the accuracy of the final model.

% Neural architecture search (NAS) dominates specialized model design under resource-constrained settings~\cite{cai2019proxylessnas, tan2019mnasnet, wu2019fbnet}.
% % Search space design is one of the key to success.
% The final accuracy highly depends on the search space design~\cite{radosavovic2020designing}. 
% Traditionally, people follow the manual model design heuristics for search space design. For example, the widely used mobile-setting search space~\cite{tan2019mnasnet, cai2019proxylessnas, wu2019fbnet, cai2020once} originates from MobileNetV2~\cite{sandler2018mobilenetv2}: they both use 224 input resolution and a similar base channel number configurations, while searching for kernel sizes, block depths, and expansion ratios. However, there lacks standard model design for microcontrollers with limited memory, so as search space design.
% % making the NAS search space design difficult. 
% One way is to manually tweak the search space for each microcontroller. However, manually tuning through trials and errors is labor intensive, making it prohibitive for a large number of deployment constraints (\eg, STM32F746 has 320kB SRAM/1MB Flash, STM32H743 has 512kB SRAM/2MB Flash, latency requirement 5FPS/10FPS).

% To address it, we propose TinyNAS, a two-stage neural architecture search method that first automatically optimizes the search space to fit the tiny and diverse resource constraints, and then performs resource-constrained model specialization to find the best model architecture.

\myparagraph{Automated search space optimization.}
We propose to optimize the search space automatically at \emph{low cost} by analyzing the computation distribution of the satisfying models.
To fit the tiny and diverse resource constraints of different microcontrollers, 
we scale the \emph{input resolution} and the \emph{width multiplier} of the mobile search space~\cite{tan2019mnasnet}. We choose from an input resolution spanning $R=\{48, 64, 80, ..., 192, 208, 224\}$  and a width multiplier $W=\{0.2, 0.3, 0.4, ..., 1.0\}$ to cover a wide spectrum of resource constraints. This leads to $12\times9=108$ possible search space configurations $S=W\times R$. Each search space configuration contains $3.3\times 10^{25}$ possible sub-networks.
Our goal is to find the best search space configuration $S^*$ that contains the model with the highest accuracy while satisfying the resource constraints.

Finding $S^*$ is non-trivial. One way is to perform neural architecture search on each of the search spaces and compare the final results. But the computation would be astronomical. Instead, 
% we hope to use a computationally light method to fast sweep over all the configurations and compare their priority. 
we evaluate the quality of the search space by randomly sampling $m$ networks from the search space and comparing the distribution of satisfying networks. 
% Specifically, we randomly sample $m$ networks from the search space and only keep the models that meet the resource limit on microcontrollers. 
Instead of collecting the Cumulative Distribution Function (CDF) of each satisfying network's \textit{accuracy}~\cite{radosavovic2019network}, which is computationally heavy due to tremendous training, we only collect the CDF of \textit{FLOPs} (see Figure~\ref{fig:cdf}). The intuition is that, within the same model family, the accuracy is usually positively related to the computation~\cite{canziani2016analysis,he2018amc}. A model with larger computation has a larger capacity, which is more likely to achieve higher accuracy. We further verify the the assumption in Section~\ref{sec:analysis}.

% can collect the accuracy of the randomly sampled networks that meet the resource constraints and plot the accuracy distribution using Cumulative Distribution Function (CDF), to compare the priority of different search space configurations. The process needs to train and get the accuracy of each sampled network, which is still intensive. We find that in the same search space family, the accuracy of sampled network is positively related to the computation (\textcolor{red}{Sec: TODO}). We instead collect the FLOPs distribution, which can be efficiently measured.

% here give an example
\input{mcunetv1/figure_text/fig_cdf}


As an example, we study the best search space for ImageNet-100 (a 100 class classification task taken from the original ImageNet) on STM32F746. We show the FLOPs distribution CDF of the top-10 search space configurations in Figure~\ref{fig:cdf}. We sample $m=1000$ networks from each space and use TinyEngine to optimize the memory scheduling for each model. We only keep the models that satisfy the memory requirement at the best scheduling. To get a quantitative evaluation of each space, we calculate the average FLOPs for each configuration
% The insight is that the design space that is more likely to produce high FLOPs models within memory constraints gives higher model capacity, thus is more likely to achieve high accuracy. 
and choose the search space with the largest average FLOPs.  For example, according to the experimental results on ImageNet-100, using the solid red space (average FLOPs 52.0M) achieves 2.3\% better accuracy compared to using the solid green space (average FLOPs 46.9M), showing the effectiveness of automated search space optimization. We will elaborate more on the ablations in Section~\ref{sec:search_space_ablation}.


\myparagraph{Resource-constrained model specialization.}
% \SH{again the first sentence should be eye catchy. you can say there are billions of IoT devices, the search cost will be prohibitive, instead, we use weight sharing (need to \textit{sell} something in this paragraph; weight sharing could be a candidate, there maybe a better one)}
% \ji{point out the difference here. }
To specialize network architecture for various microcontrollers, we need to keep a low neural architecture search cost. 
After search space optimization for each memory constraint, we perform one-shot neural architecture search~\cite{bender2018understanding, guo2019single} to efficiently find a good model, reducing the search cost by 200$\times$~\cite{cai2019proxylessnas}.  
We train one super network that contains all the possible sub-networks through \emph{weight sharing} and use it to estimate the performance of each sub-network. 
% Specifically, we first train the largest network within the optimized search space (supporting variable kernel size, expansion ratio, and block depth), and use it to initialize the super network weights. The convolution kernels are re-ranked according to their norm, so that the more important kernels have a higher priority to be used during random sampling. During training, for each batch of data, we randomly sample 4 sub-networks from the super network, and update the corresponding weights. 
We then perform evolution search to find the best model within the search space that meets the on-board resource constraints while achieving the highest accuracy. For each sampled network, we use TinyEngine to optimize the memory scheduling to measure the optimal memory usage. With such kind of co-design, we can efficiently fit the tiny memory budget. 
% We keep a population of size 100, and keep the top 20 configurations after each iteration. Then we use crossover to generate 50 new configurations from the top-20, and use mutation ($p$=0.1) to generate another 50 to form the new generation. The process is repeated by 30 times. We use TinyNAS to generate a good model architecture, and use TinyEngine to optimize the scheduling of the model and check if it satisfies the memory constraints. 
% With such co-design, our final model can fully utilize the hardware resource.  \ji{this part has limited novelty, is it too long?} \SH{too long. detalied numbers can goto exp section, or remove (such as repeat 30 times)}
% \ji{should we add more for co-design details?}
% The neural architecture search details can be found in the supplementary.
% \ji{should we elloborate more? or just leave it in supp (since the text part seems too long now)}
The details of super network training and evolution search can be found in the supplementary. 

% \subsection{System-Algorithm Co-Design}
% Describe how we co-design them

\subsection{TinyEngine: A Memory-Efficient Inference Library}
%\TODO: why code generation is better than interpreter
Researchers used to assume that using different deep learning frameworks (libraries) will only affect the  \textit{inference speed} but not the \textit{accuracy} . However, this is not the case for TinyML: the efficiency of the inference library matters a lot to both the latency and accuracy of the searched  model. Specifically, a good inference framework will make full use of the limited resources in MCU, avoiding waste of memory, and allow a larger search space for architecture search. With a larger degree of design freedom, TinyNAS is more likely to find a high accuracy model. Thus, TinyNAS is co-designed with a memory-efficient inference library, TinyEngine.
% Existing inference frameworks (\eg, TF-Lite micro, CMSIS-NN) mainly focus on the layer-level optimization with simple strategies while neglecting the model statics, which leads to potential idle resources. Meanwhile, most of them are interpreter-based and require extra memory for meta information, such as neural architecture parameters, which does not contribute much to the computation efficiency. To address this challenge, we propose a model-adaptive inference framework for TinyML, TinyEngine, that optimizes the memory scheduling and computing kernels costing the minimum hardware resource on MCU devices for a NN model as a whole.
% A deep learning model usually consists lots of layers with various configurations (e.g., operation, shapes, and so on). Therefore, each layer features different memory usage and looping behavior during inference. Existing inference frameworks like TF-Lite micro focus on optimization at layer-level but overlooks the opportunity to reduce memory usage of the whole model. We propose to generate code that consists of the optimal memory scheduling and specialized computing kernels for a given model.

\myparagraph{Code generator-based compilation.} Most existing inference libraries (\eg, TF-Lite Micro, CMSIS-NN) are interpreter-based. Though it is easy to support cross-platform development, it requires extra memory, the most expensive resource in MCU, to store the meta-information (such as model structure parameters).
% , which does not contribute much to the computation efficiency.
Instead, TinyEngine only focuses on MCU devices and adopts code generator-based compilation. It not only avoids the time for runtime interpretation, but also frees up the memory usage to allow design and inference of larger models. Compared to CMSIS-NN, TinyEngine reduced memory usage by 2.1$\times$ and improve inference efficiency by 22\% via code generation, as shown in Figures~\ref{fig:speedup} and ~\ref{fig:speedup_memory_ablation}.


\input{mcunetv1/figure_text/fig_compare_library}

\input{mcunetv1/figure_text/fig_speedup_memory_ablation}

\input{mcunetv1/figure_text/fig_binary_size}
% \input{mcunetv1/figure_text/fig_memory_ablation}

The binary size of TinyEngine is light-weight, making it very memory-efficient for MCUs. 
Unlike interpreter-based TF-Lite Micro, which prepares the code for \textit{every} operation (e.g., conv, softmax) to support cross-model inference even if they are not used, which has high redundancy. TinyEngine only compiles the operations that are used by a given model into the binary. As shown in Figure~\ref{fig:binary_size}, such model-adaptive compilation reduces code size by up to 4.5$\times$ and 5.0$\times$ compared to TF-Lite Micro and CMSIS-NN, respectively.




% TinyEngine achieves \emph{tiny memory usage} by generating inference code with the optimal scheduling memory scheduling at compile time. This eliminates runtime overheads including, memory fragmentation due to on-demand memory allocation, memory space storing information of the network architecture, and unnecessary instructions handling data movement, reducing peak memory and accelerating inference. The optimal memory scheduling allocates the minimum memory space for input and output activation and the Im2col buffer for a given model. The requirement of input and output activation is calculated based on the network architecture. For the Im2col buffer, we allocate just enough memory space to store at least one column of input data for each layer. Therefore, its size can be calculated as ${\max{kernel\_size \times input\_channels}}$ among all convolution layers in the model. There is a trade-off between buffer size and inference efficiency; increasing the buffer size potentially allows more data reuse, whereas a small buffer could lead to frequent data reload. The optimal memory scheduling allows us to reuse a column of transformed input during computing at least one output element for all channels without reloading input, minimizing peak memory while accelerating inference via substantial data reuse.
\myparagraph{Model-adaptive memory scheduling.}
% The key challenge in the TinyML is the very limited memory resources.
% Existing inference frameworks focus on the layer-level optimization with simple strategies while neglecting the model statics, which leads to potential idle resources.
% Unlike $\mu$TVM which works on SRAM only, TinyEngine leverages both SRAM and Flash memory in the MCU to support larger models. More importantly, TinyEngine reduces the memory usage by statically scheduling the memory allocation at the compilation time.
% , instead of on-demand memory allocation as in TF-Lite Micro and CMSIS.
Existing inference libraries schedule the memory for each layer solely based on the layer itself: in the very beginning, a large buffer is designated to store the input activations after im2col; when executing each layer, only one column of the transformed inputs takes up this buffer. This leads to poor input activation reuse. Instead, TinyEngine smartly adapts the memory scheduling to the model-level statistics: the \textit{maximum} memory $M$ required to fit exactly one column of transformed inputs over all the layers $\bm{L}$,
\begin{equation}
    M = \max \left( \text{kernel size}_{L_i}^2 \cdot \text{in channels}_{L_i}; \forall L_i \in \bm{L}\right).
\end{equation}
For each layer $L_j$, TinyEngine tries to tile the computation loop nests so that, as many columns can fit in that memory as possible,
\begin{equation}
    \text{tiling size of feature map width}_{L_j} = \lfloor M / \left( \text{kernel size}_{L_j}^2 \cdot \text{in channels}_{L_j}\right) \rfloor.
\end{equation}
Therefore, even for the layers with the same configuration (\eg, kernel size, \#in/out channels) in two different models, TinyEngine will provide different strategies. Such adaption fully uses the available memory and increases the input data reuse, reducing the runtime overheads including the memory fragmentation and data movement. As shown in Figure~\ref{fig:speedup_memory_ablation}, the model-adaptive im2col operation improved inference efficiency by 13\%.

\myparagraph{Computation kernel specialization.} 
% TinyEngine specialze the optimizations for different layers.
% also employs operation fusion and loop unrolling to improve the computation kernel efficiency. 
TinyEngine \textit{specializes} the kernel optimizations for different layers: loops tiling is based on the kernel size and available memory, which is different for each layer; and the inner loop unrolling is also specialized for different kernel sizes (\eg, 9 repeated code segments for 3$\times$3 kernel, and 25 for 5$\times$5 ) to eliminate the branch instruction overheads.  Operation fusion is performed for
Conv+Padding+ReLU+BN layers. These specialized optimization on the computation kernel further increased the inference efficiency by 22\%, as shown in Figure~\ref{fig:speedup_memory_ablation}.

\input{mcunetv1/figure_text/fig_inplaceDW}

\myparagraph{In-place depth-wise convolution}
We propose \textit{in-place} depth-wise convolution to further reduce peak memory. Different from standard convolutions, depth-wise convolutions do not perform filtering across channels. Therefore, once the computation of a channel is completed, the input activation of the channel can be overwritten and used to store the output activation of another channel, allowing activation of depth-wise convolutions to be updated in-place as shown in Figure~\ref{fig:inplaceDW}. This method reduces the measured memory usage by 1.6$\times$ as shown in Figure~\ref{fig:speedup_memory_ablation}.
% \myparagraph{Specialized Vectorization.} 
% TinyEngine also achieves \emph{tiny instruction overhead} at runtime, which allows larger design space under a given latency constraint. Traditionally, inference frameworks (e.g., CMSIS-NN) uses the same computing kernel with various optimization techniques to run all layers. However, such computing kernel only achieves sub-optimal performance due to lack of considering overall memory and the fact that each layer has different loop size. To address this issue, TinyEngine not only employs common optimization techniques but also specializes them for a given model. Specifically, layers (e.g., padding and convolution) are fused at compile time. Loops are tiled based on available memory, and the most inner loops are unrolled completely for each layer (e.g., 9 repeated calculations for 3$\times$3 kernel) to eliminate loop overheads. 


% \paragraph{Framework evaluation.}
% As shown in Figure~\ref{fig:speedup}, we compare the memory usage and performance of TinyEgine with existing frameworks, including $\mu$TVM, autoTVM (tuned $\mu$TVM), TF-Lite Micro, and CMSIS-NN (based on TF-Lite Micro runtime) for running common networks. The evaluation runs various models, including a tiny Cifar10 model (denoted as TinyCifar), MobileNetV2~\cite{sandler2018mobilenetv2} (denoted as MBv2), ProxylessNAS Mobile~\cite{cai2019proxylessnas} (denoted as Proxyless), and MnasNet~\cite{tan2019mnasnet} (denoted as Mnas) on a STM32F746 microcontroller. To meet the 1MB storage constraint, MBv2, Proxyless, and Mnas are respectively scaled down with 0.3, 0.3, and 0.2 width multiplier. TinyEngine achieves higher performance with much less memory usage. Compared to TF-Lite Micro, TinyEngine reduces memory usage by up to 2.6$\times$ and accelerates inference speed by 3.1$\times$. This also allows TinyNAS to find a larger model within given memory or latency constraints. 

% Furthermore, we conduct ablation study to investigate how each technique used by TinyEngine affects inference speed, as shown in Figure~\ref{fig:speedup_ablation}, which also reports average computing efficiency of each framework for running models that are executable by all frameworks except $\mu$TVM\footnote{$\mu$TVM can not run most models due to its limitation on using flash so efficiency of $\mu$TVM and autoTVM are calculated based their preliminary result compared to CMSIS-NN, as reported in ~\cite{}.}. Note that even if TinyEngine uses common optimization techniques, we still achieves performance improvement by specializing each technique at model-level, instead of at layer-level like existing frameworks.
% \input{mcunetv1/figure_text/fig_speedup}








==> mcunetv1/text/4_experiments.tex <==
\section{Experiments}

\subsection{Setups}

\myparagraph{Datasets.} 
We used 3 datasets as benchmark: ImageNet~\cite{deng2009imagenet}, Visual Wake Words (VWW)~\cite{chowdhery2019visual}, and Speech Commands (V2)~\cite{warden2018speech}. ImageNet is a standard large-scale benchmark for image classification. VWW and Speech Commands represent popular microcontroller use-cases: VWW is a vision based dataset identifying whether a person is present in the image or not; Speech Commands is an audio dataset for keyword spotting (\eg, ``Hey Siri''), requiring to classify a spoken word from a vocabulary of size 35. Both datasets reflect the always-on characteristic of microcontroller workload.
We did not use datasets like CIFAR~\cite{krizhevsky2009learning} since it is a small dataset with a limited image resolution ($32\times32$), which cannot accurately represent the benchmark model size or accuracy in real-life cases.




During neural architecture search, in order not to touch the validation set, we perform validation on a small subset of the training set (we split 10,000 samples from the training set of ImageNet, and 5,000 from VWW). Speech Commands has a separate validation\&test set, so we use the validation set for search and use the test set to report accuracy.
% \myparagraph{Training.}
The training details are in the supplementary material.



% \myparagraph{Training.}
% We train all the models using cosine learning rate, with a learning rate of 0.05 per 256 samples. On ImageNet, the largest network in the search space is trained for 150 epochs, and the super network is trained for 300 epochs. We reduces the training schedule by half on other datasets. 
% We first train the super network using the best search space under each setting. Following~\cite{cai2020once}, we first train the largest network in the space and use it as the initial weight for the super network to accelerate convergence. The super network is trained for 300 epochs for ImageNet and 150 epochs for other datasets. We then use evolution search to find the models that achieve the best accuracy under the given constraints. \textbf{TODO: needs more details here}


\myparagraph{Model deployment.} 
We perform int8 linear quantization to deploy the model.
% , the industrial standard to reduce model size. 
% It can be done without fine-tuning at negligible accuracy loss.
We deploy the models on microcontrollers of diverse hardware resource, including STM32F412 (Cortex-M4, 256kB SRAM/1MB Flash), STM32F746 (Cortex-M7, 320kB/1MB Flash), STM32F765 (Cortex-M7, 512kB SRAM/1MB Flash), and STM32H743 (Cortex-M7, 512kB SRAM/2MB Flash). 
% All the MCU results  are reported on STM32F746 MCU (320kB SRAM/1MB Flash), except for the OOM results that are measured on a larger MCU: STM32H743 (512kB SRAM/2MB Flash). 
By default, we use STM32F746 to report the results unless otherwise specified.
All the latency is normalized to STM32F746 with 216MHz CPU. 

% \myparagraph{Search Space.}
% We first run statistically search space optimization to find a good search space under SRAM, Flash and latency constraints. We used the same search space as in~\cite{tan2019mnasnet, cai2019proxylessnas} and follow~\cite{cai2020once} to support variable input resolution (span over 48), variable depth per block (2/3/4) and variable expansion ratio (3/4/5/6) for each block.
% We scale the search space by adjusting the input resolution range (choosing from \{48-64, 64-80, ..., 128-176\})
%  and the network base width multiplier (choosing from \{0.2, 0.3, ..., 0.8\}). We randomly sampled 5,000 network architectures from the space to evaluate the statistics. The combination leads to $6\times7=42$ possible search spaces.






\subsection{Large-Scale Image Recognition on Tiny Devices}




With our system-algorithm co-design, we achieve record high accuracy (70.7\%) on large-scale ImageNet recognition on microcontrollers. 
% We test our algorithm on two widely used microcontrollers STM32F746 (320kB SRAM, 1MB Flash) and STM32743 (512kB SRAM, 2MB Flash). 
We co-optimize TinyNAS and TinyEngine to find the best runnable network.
We compare our results to several baselines. We generate the \emph{best scaling} of MobileNetV2~\cite{sandler2018mobilenetv2} (denoted as \textbf{S-MbV2}) and ProxylessNAS Mobile~\cite{cai2019proxylessnas} (denoted as \textbf{S-Proxyless}) by compound scaling down the width multiplier and the input resolution until they meet the memory requirement. We train and evaluate the performance of all the satisfying scaled-down models on the Pareto front \footnote{\eg, if we have two models (w0.5, r128) and (w0.5, r144) meeting the constraints, we only train and evaluate (w0.5, r144) since it is strictly better than the other; if we have two models (w0.5, r128) and (w0.4, r144) that fits the requirement, we train both networks and report the higher accuracy.}, and then report the highest accuracy as the baseline.
The former is an efficient manually designed model, the latter is a state-of-the-art NAS model. We did not use MobileNetV3~\cite{howard2019searching}-alike models because the hard-swish activation is not efficiently supported on microcontrollers.  
% We follow~\cite{chowdhery2019visual} to shrink the last convolutional layer in MobileNetV2, otherwise the classifier will take >1MB (weight of shape $1280\times1000$), exceeding memory constraints. 

\input{mcunetv1/figure_text/tab_codesign}
\input{mcunetv1/figure_text/tab_4bit}
\input{mcunetv1/figure_text/fig_compare_resnet18}

\myparagraph{Co-design brings better performance.}


Both the inference library and the model design help to fit the resource constraints of microcontrollers. 
As shown in Table~\ref{tab:codesign}, when running on a tight budget of 320kB SRAM and 1MB Flash, the optimal scaling of MobileNetV2 and ProxylessNAS models only achieve 35.2\% and 49.5\% top-1 accuracy on ImageNe using CMSIS-NN~\cite{lai2018cmsis}. With TinyEngine, we can fit larger models that achieve higher accuracy of 47.4\% and 56.4\%; with TinyNAS, we can specialize a more accurate model under the tight memory constraints to achieve 55.5\% top-1 accuracy. Finally, with system-algorithm co-design, MCUNet further advances the accuracy to 61.8\%, showing the advantage of joint optimization.

Co-design improves the performance at various latency constraints (Table~\ref{tab:latency_imagenet}). TinyEngine accelerates inference to achieve higher accuracy at the same latency constraints. For the optimal scaling of MobileNetV2, TinyEngine improves the accuracy by 1.9\% at 5 FPS setting and 5.4\% at 10 FPS. With MCUNet co-design, we can further improve the performance by 8.3\% and 6.4\%. 


\myparagraph{Diverse hardware constraints \& lower bit precision.} 

We used int8 linear quantization for both weights and activations, as it is the industrial standard for faster inference and usually has negligible accuracy loss without fine-tuning.
% As the microcontroller only supports 16-bit instructions, the multiplication operands are converted to 16-bit, and accumulated in 32bit.
We also performed 4-bit linear quantization on ImageNet, which can fit larger number parameters. The results are shown in Table~\ref{tab:4bit}.
% and it is easy to use, usually preserving the accuracy without fine-tuning. 
% ; using a lower bit does not bring acceleration.
% As shown in~\cite{rusci2019memory}, using a lower and mixed bit precision (8/4/2-bit) helps to improve the accuracy-memory trade-off on microcontrollers. Therefore, we also study a more aggressive quantization scheme using 4-bit quantization (weights and activation) to reduce memory footprint. 
MCUNet can handle diverse hardware resources on different MCUs with Cortex-M4 (F412) and M7 (F746, F765, H743) core.
% Under the same memory constraints, 4-bit MCUNet outperforms 8-bit by 2.2\% by fitting a larger model in the memory.
Without mixed-precision, we can already outperform the existing state-of-the-art~\cite{rusci2019memory} on microcontrollers, showing the effectiveness of system-algorithm co-design. We believe that we can further advance the Pareto curve in the future with mixed precision quantization. 

Notably, our model achieves a record ImageNet top-1 accuracy of $70.7\%$ on STM32H743 MCU. To the best of our knowledge, we are the first to achieve $>70\%$ ImageNet accuracy on off-the-shelf commercial microcontrollers. Compared to ResNet-18 and MobileNetV2-0.75 (both in 8-bit) which achieve a similar ImageNet accuracy (69.8\%), our MCUNet reduces the the memory usage by 3.5$\times$ and the Flash usage by 5.7$\times$  (Figure~\ref{fig:compare_resnet18}) to fit the tiny memory size on microcontrollers.
 
\subsection{Visual\&Audio Wake Words}


\input{mcunetv1/figure_text/fig_vww_curve}
\input{mcunetv1/figure_text/fig_gcommands_curve}

We benchmarked the performance on two wake words datasets: Visual Wake Words~\cite{chowdhery2019visual} (VWW) and Google Speech Commands (denoted as GSC) to compare the accuracy-latency and accuracy-peak memory trade-off. We compared to the optimally scaled MobileNetV2 and ProxylessNAS running on TF-Lite Micro.  The results are shown in Figure~\ref{fig:vww_curve}. MCUNet significantly advances the Pareto curve. On VWW dataset, we can achieve higher accuracy at 2.4-3.4$\times$ faster inference speed and 3.7$\times$ smaller peak memory. We also compare our results to the previous first-place solution on VWW challenge~\cite{vww_first_place} (denoted as Han \etal). We scaled the input resolution to tightly fit the memory constraints of 320kB and re-trained it under the same setting like ours. We find that MCUNet achieves 2.4$\times$ faster inference speed compared to the previous state-of-the-art. Interestingly, the model from~\cite{vww_first_place} has a much smaller peak memory usage compared to the biggest MobileNetV2 and ProxylessNAS model, while having a higher computation and latency. It also shows that a smaller peak memory is the key to success on microcontrollers.

On the Speech Commands dataset, MCUNet achieves a higher accuracy at 2.8$\times$ faster inference speed and $4.1\times$ smaller peak memory. It achieves 2\% higher accuracy compared to the largest MobileNetV2, and 3.3\% improvement compared to the largest runnable ProxylessNAS under 256kB SRAM constraint. 

\subsection{Object Detection on MCUs}

\input{mcunetv1/figure_text/tab_detection}
To show the generalization ability of MCUNet framework across different tasks, we apply MCUNet to object detection.
Object detection is particularly challenging for memory-limited MCUs: a high-resolution input is usually required to detect the relatively small objects, which will increase the peak performance significantly. We benchmark the object detection performance of our MCUNet and scaled MobileNetV2+CMSIS-NN on  on Pascal VOC~\cite{everingham2010pascal} dataset. We used YOLOv2~\cite{redmon2017yolo9000} as the detector; other more advanced detectors like YOLOv3~\cite{redmon2018yolov3} use multi-scale feature maps to generate the final prediction, which has to keep intermediate activations in the SRAM, increasing the peak memory by a large margin. The results on H743 are shown in Table~\ref{tab:detection}. Under tight memory budget (only 512kB SRAM and 2MB Flash), MCUNet significantly improves the mAP by 20\%, which makes AIoT applications more accessible.





\subsection{Analysis}
\label{sec:analysis}


\vspace{-8pt}
\paragraph{Search space optimization matters.}
\label{sec:search_space_ablation}
Search space optimization significantly improves the NAS accuracy. We performed an ablation study on ImageNet-100, a subset of ImageNet with 100 randomly sampled categories. The distribution of the top-10 search spaces is shown in Figure~\ref{fig:cdf}. We sample several search spaces from the top-10 search spaces and perform the whole neural architecture search process to find the best model inside the space that can fit 320kB SRAM/1MB Flash.

\input{mcunetv1/figure_text/tab_fig_spaces}

We compare the accuracy of the searched model using different search spaces in Table~\ref{tab:acc_vs_space}. Using the search space configuration found by our algorithm, we can achieve 78.7\% top-1 accuracy, closer to ResNet-18 on 224 resolution input (which runs out of memory). We evaluate several randomly sampled search spaces from the top-10 spaces; they perform significantly worse. Another baseline is to use a very large search space supporting variable resolution (96-176) and variable width multipliers (0.3-0.7). Note that this ``huge space'' 
% is actually much smaller than the  space scope we used (48-224 resolution, 0.2-1.0 width multiplier), and also 
contains the best space. However, it fails to get good performance. We hypothesize that using a super large space increases the difficulty of training super network and evolution search.
We plot the relationship between the accuracy of the final searched model and the mean FLOPs of the search space configuration in Figure~\ref{fig:acc_vs_auc}. We can see a clear positive relationship, which backs our algorithm.


% \myparagraph{System/DL Co-Design is necessary}
% Evaluate the OP/s or arithmetic intensity during evolution search, using different system.

\myparagraph{Sensitivity analysis on search space optimization.}
\input{mcunetv1/figure_text/fig_grid_config}
We inspect the results of search space optimization and find some interesting patterns. The results are shown in Figure~\ref{fig:grid_config}. We vary the SRAM limit from 192kB to 512kB and Flash limit from 512kB to 2MB, and show the chosen width multiplier and resolution. Generally, with a larger SRAM to store a larger activation map, we can use  a higher input resolution; with a larger Flash to store a larger model. we can use a larger width multiplier. When we increase the SRAM and keep the Flash from point 1 to point 2 (\textcolor{mydarkred}{red rectangles}), the width is not increased as Flash is small; the resolution increases as the larger SRAM can host a larger activation. From point 1 to 3, the width increases, and the resolution actually decreases. This is because a larger Flash hosts a wider model, but we need to scale down the resolution to fit the small SRAM.
Such kind of patterns is non-trivial and hard to discover manually.

\myparagraph{Evolution search. }
\input{mcunetv1/figure_text/fig_evolution_curve}
The curve of evolution search on different inference library is in Figure~\ref{fig:evolution_curve}. The solid line represents the average value, while the shadow shows the range of (min, max) accuracy. On TinyEngine, evolution clearly outperforms random search, with 1\% higher best accuracy. The evolution on CMSIS-NN leads to much worse results due to memory inefficiency: the library can only host a smaller model compared to TinyEngine, which leads to lower accuracy.


% \myparagraph{Accuracy \vs FLOPs. }
% % \input{mcunetv1/figure_text/fig_acc_flops}
% We analyze the assumption that accuracy is positively related to computation in the same model family on ImageNet-100. We randomly sample 1000 networks from different search spaces and plot the accuracy. We use the same color for all the points in the same search space. The distribution is shown in Figure~\ref{fig:acc_flops}. We cam see a clear positive relationship.



% \myparagraph{Arithmetic Intensity}


==> mcunetv1/text/5_conclusion.tex <==
% \vspace{-5pt}
\section{Conclusion}
\vspace{-5pt}
We propose MCUNet to jointly design the neural network architecture (TinyNAS) and the inference library (TinyEngine), enabling deep learning on tiny hardware resources. We achieved a record ImageNet accuracy (70.7\%) on off-the-shelf microcontrollers, and accelerated the inference of wake word applications by 2.4-3.4$\times$.  Our study suggests that the era of always-on tiny machine learning on IoT devices has arrived.


\newpage


\section*{Statement of Broader Impacts}

Our work is expected to enable tiny-scale deep learning on microcontrollers and further democratize deep learning applications. Over the years, people have brought down the cost of deep learning inference from \$5,000 workstation GPU to \$500 mobile phones. We now bring deep learning to microcontrollers costing \$5 or even less, which greatly expands the scope of AI applications, making AI much more accessible. 

Thanks to the low cost and large quantity (250B) of commercial microcontrollers, we can bring AI applications to every aspect of our daily life, including personalized healthcare, smart retail, precision agriculture, smart factory, \etc. People from rural and under-developed areas without Internet or high-end hardware can also enjoy the benefits of AI. 
Our method also helps combat COVID-19 by providing affordable deep learning solutions  detecting face masks and people gathering on edge devices without sacrificing privacy.

With these always-on low-power microcontrollers, we can process raw sensor data right at the source.
% so that we only need to store/transfer the useful information. 
It helps to protect privacy since data no longer has to be transmitted to the cloud but processed locally.  % \ji{seesm like a separate point... should we remove?}


\section*{Acknowledgments}
We thank MIT Satori cluster for providing the computation resource. We thank MIT-IBM Watson AI Lab, Qualcomm, NSF CAREER Award \#1943349 and NSF RAPID Award \#2027266 for supporting this research.


% One possible negative impact could be due to the wider adoption of deep learning algorithms, leading to potential social problems like privacy and bias.

% We will open-source both the efficient inference library TinyEngine and the TinyNAS algorithm, which will benefit the edge AI community. 
% We hope with joint effort, we can enjoy the benefit of tiny deep learning without the negative impacts. 





==> mcunetv2/figure_text/fig_analytic_mem_flops.tex <==

\begin{figure*}[t]
    \centering
     \includegraphics[width=1.0\textwidth]{mcunetv2/figures/analytic_mem_flops_abs2.pdf}
     % \vspace{-10pt}
    \caption{\textbf{Analytical profiling}: patch-based inference significantly reduces the inference peak memory by \textbf{3.7-8.0$\times$} at a small computation overhead of 8-17\%. The memory reduction and computation overhead are related to the network design. For MobileNetV2, we can reduce the computation overhead from 10\% to 3\% by redistributing the receptive field. All networks take an input resolution of $224^2$ and $4\times4$ patches. 
    }
    \label{fig:analytic_mem_flops}
\end{figure*}



\begin{figure*}[t]
    \centering
     \includegraphics[width=1.0\textwidth]{mcunetv2/figures/ondevice_mem_flops3.pdf}
     % \vspace{-10pt}
    \caption{\textbf{On-device measurement}: patch-based inference reduce the \emph{measured} peak SRAM usage by \textbf{4-6$\times$} when running on MCUs. The latency overhead could be large for some networks, but we can reduce it to 4\% with proper architecture design (MbV2-RD).
    We scale down width $w$ and resolution to fit MCU memory.
    }
    \label{fig:ondevice_mem_flops}
\end{figure*}

==> mcunetv2/figure_text/fig_granularity_study.tex <==

\begin{figure*}[t]
    \centering
     \includegraphics[width=1.0\textwidth]{mcunetv2/figures/granularity_study2_eps.pdf}
    \caption{Ablation study on patch-based inference. \textbf{Left}: the peak memory generally goes down with more blocks being executed patch-by-patch ($n$) and a larger patch number ($p$).
    The optimal index for MobileNetV2 is $n^*=5$, where the feature map is down-sampled by 8$\times$. \textbf{Right}: splitting the input images into more patches (larger $p$) leads to larger computation overhead. Receptive field redistribution reduces the overhead (MbV2-RD). 
    }
    \label{fig:granularity_study}
\end{figure*}

==> mcunetv2/figure_text/tab_compare_nas.tex <==
\begin{table}[h]
    \caption{Our NAS method outperforms existing state-of-the-art tiny networks in terms of computation-accuracy trade-off, especially under tiny computation settings (<50M). All our models are derived from \emph{the same search space}, while obtaining the best accuracy at different budgets.
    For models with \textcolor{red}{*}, we re-measure the MACs and parameters using our profiler.  }
    \label{tab:compare_nas}
    \centering
    \small{
     \begin{tabular}{lllcccc}
    \toprule
  Budget & Model & Setting & MACs & Weights & Top-1  & Top-5 \\  
  \midrule
\multirow{2}{*}{\shortstack{100M\\MACs}} & MobileNetV1 0.5$\times$ (r=192)~\cite{howard2017mobilenets} & Manual+Scale & 110M & 1.3M & 61.7\% & 83.6\% \\
& MobileNetV2 0.75$\times$(r=160)~\cite{sandler2018mobilenetv2} & Manual+Scale & 107M & 2.6M & 66.4\% & 87.3\%  \\
& MobileNetV3 Small 1.25$\times$~\cite{howard2019searching} & NAS+Scale & 91M & 3.6M & 70.4\% & - \\
& EfficientNet-B\textsuperscript{-2}~\cite{tan2019efficientnet,han2020model} & NAS+Scale & 98M & 3.0M & 70.5\% & 89.5\% \\
& TinyNet-C~\cite{han2020model}  \textcolor{red}{*} & NAS+Scale & 103M & 2.5M & 71.2\% & 89.7\% \\
 \cmidrule{2-7}
 & Ours (uniform $w$) & Joint Search & 98M & 4.2M & \textbf{72.3\%} & \textbf{90.6\%} \\ 
 & Ours (flexible $w$) & Joint Search & 99M & 3.9M & \textbf{72.3\%} & 90.5\% \\
\midrule
\multirow{2}{*}{\shortstack{50M\\MACs}} & MobileNetV2 0.35$\times$~\cite{sandler2018mobilenetv2} & Manual+Scale & 59M & 1.7M & 60.3\% & 82.9\%\\
 & MnasNet-A1 0.35$\times$~\cite{tan2019mnasnet} & NAS+Scale & 63M & 1.7M & 64.1\% & 85.1\% \\ 
& MnasNet-search1~\cite{tan2019mnasnet} & NAS & 65M & 1.9M &  64.9\% & - \\ 
& EfficientNet-B\textsuperscript{-3}~\cite{tan2019efficientnet,han2020model} & NAS+Scale & 51M & 2.0M & 65.0\% & 85.2\% \\
& TinyNet-D~\cite{han2020model} \textcolor{red}{*} & NAS+Scale & 53M & 2.3M & 67.0\% & 87.1\%\\
& MobileNetV3 Small 1.0$\times$~\cite{howard2019searching} & NAS & 56M & 2.5M & 67.4\% & -\\  %
 \cmidrule{2-7}
 & Ours (uniform $w$) & Joint Search & 50M & 2.8M & 67.9\% & 87.7\% \\
 & Ours (flexible $w$) & Joint Search & 50M & 3.5M & \textbf{68.8\%} & \textbf{88.2\%}\\
\midrule
\multirow{2}{*}{\shortstack{25M\\MACs}} & MobileNetV2 0.35$\times$ (r=160)~\cite{sandler2018mobilenetv2} & Manual+Scale &  30M & 1.7M & 55.7\% & 79.1\% \\
 & MnasNet-A1 0.57$\times$ (r=128)~\cite{tan2019mnasnet} & NAS+Scale & 22M & 1.7M & 54.8\% & 78.1\% \\
 & EfficientNet-B\textsuperscript{-4}~\cite{tan2019efficientnet,han2020model} & NAS+Scale & 24M & 1.3M & 56.7\% & 79.8\% \\ 
 & MobileNetV3 Small 0.5$\times$~\cite{howard2019searching} & NAS+Scale & 23M & 1.6M & 58.0\% & - \\
 & TinyNet-E~\cite{han2020model} \textcolor{red}{*} & NAS+Scale & 25M & 2.0M & 59.9\% & 81.1\% \\ 
  \cmidrule{2-7}
 & Ours (uniform $w$) & Joint Search & 25M & 2.6M & 63.2\% & 84.7\% \\
 & Ours (flexble $w$) & Joint Search & 25M & 3.2M & \textbf{63.9\%} & \textbf{84.9\%} \\ 
    \bottomrule
     \end{tabular}
     }
\end{table}

==> mcunetv2/figure_text/tab_compare_other_method.tex <==
\renewcommand \arraystretch{0.9}
\begin{table*}[t]
    \setlength{\tabcolsep}{4pt}
    \caption{Comparing \method with other memory-saving methods. Non-overlapping patches suffer from a degraded detection performance; RNNPool~\cite{saha2020rnnpool} leads to worse performance and slower training time. \method with redistributed model maintains the accuracy at the same training cost. Degraded items marked in \textcolor{red}{red}.}
    \label{tab:compare_methods}
    \centering
    \small{
     \begin{tabular}{llccccc}
    \toprule
  Model & Inference & Invariant  & Peak Mem\textsubscript{\texttt{fp32}}  & 
 Train time
  &   ImgNet Top-1 & VOC mAP  \\  
    \midrule
    MbV2~\cite{sandler2018mobilenetv2}
    & Per-layer& \ding{51}   & 2.29MB &  1.0$\times$ &  72.2\% & 75.4\% \\
    \midrule
    Non-overlap & Per-patch  & \textcolor{red}{\ding{55}} & \textbf{0.19MB} & 1.0$\times$ & 71.8\% & \textcolor{red}{73.9\%}\\  %
    MbV2-RNNPool~\cite{saha2020rnnpool} & Streaming & \textcolor{red}{\ding{55}} &  0.24MB & \textcolor{red}{3.2$\times$} & \textcolor{red}{70.1\%} & \textcolor{red}{71.0\%} \\ %
    MbV2-RD (ours) & Per-patch  & \ding{51} &   \textbf{0.19MB} & 1.0$\times$ & 72.1\% & 75.7\%
    \\
    \bottomrule
     \end{tabular}
     }
\end{table*}


==> mcunetv2/figure_text/tab_network_redistribute.tex <==
\renewcommand \arraystretch{0.9}
\begin{table*}[t]
    \setlength{\tabcolsep}{3.5pt}
    \caption{Per-patch inference reduces the peak memory by 8$\times$ for MobileNetV2~\cite{sandler2018mobilenetv2} (1372kB to 172kB), but it increases the overall computation by 10\% due to patch overlapping. 
    We futher propose receptive field redistribution (MbV2-RD) which reduces the overall overhead to only 3\% without hurting performance.
    }
    \vspace{5pt}
    \label{tab:network_redistribution}
    \centering
    \small{
     \begin{tabular}{lccccccccc}
    \toprule
  \multirow{2}{*}{Model} &  \multirow{2}{*}{\shortstack{Patch\\Size}} & \multicolumn{2}{c}{Comp. overhead} & \multicolumn{2}{c}{MACs\textsubscript{(4$\times$4 patches)}}  & \multicolumn{2}{c}{Peak SRAM} &   \multirow{2}{*}{\shortstack{ImgNet\\Top-1}} & \multirow{2}{*}{\shortstack{VOC\\mAP}}  \\  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
  & & patch-stage & overall &patch-stage & overall & per-layer & per-patch \\ 
    \midrule
   MbV2~\cite{sandler2018mobilenetv2} & $75^2$ & +42\% & +10\% & 130M & 330M & 1372kB & 172kB (\textbf{8$\times$$\downarrow$}) & 72.2\%  & 75.4\% \\ 
    MbV2-RD   & $63^2$ & +18\% & +3\%  & 73M & 301M  & 1372kB &  172kB (\textbf{8$\times$$\downarrow$}) &   72.1\% & 75.7\%
    \\
    \bottomrule
     \end{tabular}
     }
     % \vspace{-15pt}
\end{table*}







==> mcunetv2/main.tex <==

\def\method{MCUNetV2\xspace}

\input{mcunetv2/text/0_abstract}
\input{mcunetv2/text/1_introduction}
\input{mcunetv2/text/3_approach}
\input{mcunetv2/text/4_experiments}
\input{mcunetv2/text/2_related_work}
\input{mcunetv2/text/5_conclusion}



==> mcunetv2/text/0_abstract.tex <==
\begin{abstract}
Tiny deep learning on microcontroller units (MCUs) is challenging due to the limited memory size. %
We find that the memory bottleneck is due to the \emph{imbalanced memory distribution} in convolutional neural network (CNN) designs: the first several blocks have an order of magnitude larger memory usage than the rest of the network. To alleviate this issue, we propose a generic \emph{patch-by-patch} inference scheduling, which operates only on a small spatial region of the feature map and significantly cuts down the peak memory. 
However, naive implementation brings overlapping patches and computation overhead. We further propose \emph{receptive field redistribution} to shift the receptive field and FLOPs to the later stage and reduce the computation overhead.
Manually redistributing the receptive field is difficult. We automate the process
with neural architecture search to jointly optimize the neural architecture and inference scheduling, leading to \method.
Patch-based inference effectively reduces the peak memory usage of existing networks by 4-8$\times$. Co-designed with neural networks, \method sets a record ImageNet accuracy on MCU (71.8\%), and achieves >90\% accuracy on the visual wake words dataset under only 32kB SRAM. \method also unblocks object detection on tiny devices, achieving 16.9\% higher mAP on Pascal VOC compared to the state-of-the-art result. Our study largely addressed the memory bottleneck in tinyML and paved the way for various vision applications beyond image classification.




\end{abstract}

==> mcunetv2/text/1_introduction.tex <==
\section{Introduction}





IoT devices based on tiny hardware like microcontroller units (MCUs) are ubiquitous nowadays. Deploying deep learning models on such tiny hardware will enable us to democratize artificial intelligence.
However, tiny deep learning is fundamentally different from mobile deep learning due to the tight memory budget~\cite{lin2020mcunet}:
a common MCU usually has an SRAM smaller than 512kB, which is too small for deploying most off-the-shelf deep learning networks.
Even for more powerful hardware like Raspberry Pi 4, fitting inference into the L2 cache (1MB) can significantly improve energy efficiency.
These pose new challenges to efficient AI inference with a small peak memory usage.


Existing work employs pruning~\cite{han2016deep, he2018amc, he2017channel, liu2017learning, liu2019metapruning}, quantization~\cite{han2016deep, zhu2016trained, zhou2016dorefa, rastegari2016xnor, wang2019haq, choi2018pact, rusci2019memory}, and neural architecture search~\cite{cai2019proxylessnas, tan2019mnasnet, wu2019fbnet, cai2020once} for efficient deep learning.
However, these methods focus on reducing the number of parameters and FLOPs, but not the memory bottleneck. The tight memory budget limits the feature map/activation size, restricting us to use a small model capacity or a small input image size. 
Actually, the input resolutions used in existing tinyML work are usually small ($<224^2$)~\cite{lin2020mcunet}, which might be acceptable for image classification (\eg, ImageNet~\cite{deng2009imagenet}, VWW~\cite{chowdhery2019visual}), but not for dense prediction tasks like objection detection: as in Figure~\ref{fig:cls_det_degrade}, the performance of object detection degrades much faster with input resolution than image classification. 
Such a restriction hinders the application of tiny deep learning on many real-life tasks (\eg, person detection). 

\input{mcunetv2/figure_text/fig_mbv2_mem}



\begin{figure}[t]
    \centering
     \includegraphics[width=0.28\textwidth]{mcunetv2/figures/cls_det_degrade3.pdf}
    \caption{Detection is more sensitive to smaller resolutions. }
    \label{fig:cls_det_degrade}
\end{figure}


We perform an in-depth analysis on memory usage of each layer in efficient network designs and find that they have a very \emph{imbalanced activation memory distribution}. Take MobileNetV2~\cite{sandler2018mobilenetv2} as an example, as shown in Figure~\ref{fig:mbv2_mem}, only the first 5 blocks have a high peak memory (>450kB), becoming the memory bottleneck of the entire network. The remaining 13 blocks have a low memory usage, which can easily fit a 256kB MCU.
The peak memory of the initial memory-intensive stage is $8\times$ higher than the rest of the network. Such a memory pattern leaves a huge room for optimization: if we can find a way to ``bypass'' the memory-intensive stage, we can reduce the overall peak memory by $8\times$. %


In this paper, we propose \method to address the challenge. We first propose a patch-by-patch execution order for the initial memory-intensive stage of CNNs (Figure~\ref{fig:spatial_partial}). Unlike conventional layer-by-layer execution, it operates on a small spatial region of the feature map at a time, instead of the whole activation. Since we only need to store the feature of a small patch, we can significantly cut down the peak memory of the initial stage (blue to yellow in Figure~\ref{fig:spatial_partial}), allowing us to fit a larger input resolution. However, the reduced peak memory comes at the price of computation overhead:
in order to compute the non-overlapping output patches, the input image patches need to be overlapped (Figure~\ref{fig:spatial_partial}(b)), leading to repeated computation. 
The overhead is positively related to the receptive field of the initial stage: the larger the receptive field, the larger the input patches, which leads to more overlapping.
We further propose \emph{receptive field redistribution} to shift the receptive field and workload to the later stage of the network. This reduces the patch size as well as the computation overhead caused by overlapping, without hurting the performance of the network. 
Finally, patch-based inference brings a larger design space for the neural network, giving us more freedom trading-off input resolution, model size, \etc.
We also need to minimize the computation overhead under patch-based execution. To explore such a large and entangled space, we propose to jointly design the optimal deep model and its inference schedule with neural architecture search given a specific dataset and hardware.

Patch-based inference effectively reduces the peak memory usage of existing networks by 4-8$\times$ (Figure~\ref{fig:analytic_mem_flops}). The results are further improved when co-designing neural architecture with inference scheduling. On ImageNet~\cite{deng2009imagenet}, we achieve a record accuracy of 71.8\% on MCU (Table~\ref{tab:mcu_imagenet}); on visual wake words dataset~\cite{chowdhery2019visual}, we are able to achieve >90\% accuracy under only 32kB SRAM, which is 4.0$\times$ smaller compared to MCUNetV1~\cite{lin2020mcunet}, greatly lowering the boundary of tiny deep learning (Figure~\ref{fig:vww_curves}). \method further unlocks the possibility to perform dense prediction tasks on MCUs (\eg, object detection), which was not practical due to the limited input resolution.  
We are able to achieve 64.6\% mAP under 256kB SRAM constraints and 68.3\% under 512kB, which is 16.9\% higher compared to the existing state-of-the-art solution, making object detection applicable on a tiny ARM Cortex-M4 MCU. 
Our contributions can be summarized as follows:
\begin{itemize}[leftmargin=*]
\item We systematically analyze the memory usage pattern of efficient CNN designs and find that they suffer from a \emph{imbalanced memory distribution}, leaving a huge room for optimization.
\item We propose a patch-based inference scheduling to significantly reduce the peak memory required for running CNN models, 
together with receptive field redistribution to minimize the computation overhead.

\item With the joint design of network architecture and inference scheduling, we achieve a record performance for tiny image classification and objection detection on MCUs. 
Our work largely addressed the memory bottleneck for tinyML, paving the way for various vision applications.
\end{itemize}











==> mcunetv2/text/2_related_work.tex <==
\section{Related Work}



\myparagraph{Tiny deep learning on microcontrollers.}
Deploying deep learning models on memory-constrained microcontrollers requires an efficient inference framework and model architecture. Existing deployment frameworks include TensorFlow Lite Micro~\cite{abadi2016tensorflow}, CMSIS-NN~\cite{lai2018cmsis}, TinyEngine~\cite{lin2020mcunet}, MicroTVM~\cite{chen2018tvm}, CMix-NN~\cite{capotondi2020cmix}, \etc. However, all of the above frameworks support only \emph{per-layer} inference, which limits the model capacity executable under a small memory and makes higher resolution input impossible. %

\myparagraph{Efficient neural network.}
For efficient deep learning, people apply pruning~\cite{han2016deep, he2018amc, lin2017runtime, he2017channel, liu2017learning, liu2019metapruning} and quantization~\cite{han2016deep, zhu2016trained, zhou2016dorefa, rastegari2016xnor, wang2019haq, choi2018pact, rusci2019memory, langroudi2021tent} to compress an off-the-shelf deep network, or directly design an efficient network architecture~\cite{howard2017mobilenets, sandler2018mobilenetv2, howard2019searching, ma2018shufflenet, zhang2018shufflenet}. Neural architecture search (NAS)~\cite{zoph2017neural, zoph2018learning, liu2019darts, cai2019proxylessnas, tan2019mnasnet, wu2019fbnet} can design efficient models in an automated way. It has been used to improve 
tinyML on MCUs~\cite{lin2020mcunet, banbury2021micronets, liberis2020mu, fedorov2019sparse, lyu2021resource}. 
However, most of the NAS methods use the conventional hierarchy CNN backbone design, which leads to an imbalanced memory distribution under per-layer inference (Section~\ref{sec:understand}), restricting the input resolution. Therefore, they are not able to achieve good performance on tasks like object detection without our patch-based inference scheduling. %


\myparagraph{Computation scheduling/re-ordering.}
The memory requirement to run a deep neural network is related to the implementation. It is possible to reduce the required memory by optimizing the convolution loop-nest~\cite{stoutchinin2019optimally}, reordering the operator executions~\cite{liberis2019neural, ahn2020ordering}, or temporarily swapping data off SRAM~\cite{miao2021enabling}.
Computing partial spatial regions across multiple layers can reduce the peak memory~\cite{goetschalckx2019breaking,alwani2016fused, saha2020rnnpool}. 
However, system-only optimization leads to either large repeated computation or a highly complicated dataflow.
Our work explores joint system and model optimization to reduce the peak memory at a negligible computation overhead while still allowing conventional convolution optimization techniques like im2col, tiling, \etc. 







==> mcunetv2/text/3_approach.tex <==


\section{Understanding the Memory Bottleneck of Tiny Deep Learning}
\label{sec:understand}





We systematically analyze the memory bottleneck of CNN models.

\myparagraph{Imbalanced memory distribution.}
As an example, we provide the per-block peak memory usage of MobileNetV2~\cite{sandler2018mobilenetv2} in Figure~\ref{fig:mbv2_mem}. The profiling is done in \texttt{int8} (details in Section~\ref{sec:mem_profile}). 
We can observe a clear pattern of \emph{imbalanced memory usage distribution}. The first 5 blocks have large peak memory, exceeding the memory constraints of MCUs, while the remaining 13 blocks easily fit 256kB memory constraints. The third block has $8\times$ larger memory usage than the rest of the network, becoming the memory bottleneck.
We also inspect other efficient network designs and find the phenomenon quite common across different CNN backbones, even for models specialized for memory-limited microcontrollers~\cite{lin2020mcunet}. The detailed statistics are provided in the supplementary. 


We find that this situation applies to most single-branch or residual CNN designs due to the hierarchical structure\footnote{some CNN designs have highly complicated branching structure (\eg, NASNet~\cite{zoph2018learning}), but they are generally less efficient for inference~\cite{ma2018shufflenet, tan2019mnasnet, cai2019proxylessnas}; thus not widely used for edge computing.}: after each stage, the image resolution is down-sampled by half, leading to 4$\times$ fewer pixels, while the channel number increases only by 2$\times$~\cite{simonyan2014very, he2016deep, howard2017mobilenets} or by an even smaller ratio~\cite{sandler2018mobilenetv2, howard2019searching, tan2019efficientnet}, resulting in a decreasing activation size. Therefore, the memory bottleneck tends to appear at the early stage of the network, after which the peak memory usage is much smaller. 
\myparagraph{Challenges and opportunities.}
The imbalanced memory distribution significantly limits the model capacity and input resolution executable on MCUs. 
In order to accommodate the initial memory-intensive stage, the whole network needs to be scaled down even though the majority of the network already has a small memory usage.
It also makes resolution-sensitive tasks (\eg, object detection) difficult, as a high-resolution input will lead to large initial peak memory. Consider the first convolutional layer in MobileNetV2~\cite{sandler2018mobilenetv2} with input channels 3, output channels 32, and stride 2, running it on an image of resolution $224\times224$ requires a memory of $3\times224^2+32\times112^2=539 \text{kB}$ even when quantized in \texttt{int8}, which cannot be fitted into microcontrollers.
On the other hand, if we can find a way to ``bypass'' the initial memory-intensive stage, we can greatly reduce the peak memory of the whole network, leaving us a large room for optimization.



\section{\method: Memory-Efficient Patch-based Inference}


\subsection{Breaking the Memory Bottleneck with Patch-based Inference}
\input{mcunetv2/figure_text/fig_spatial_partial}

We propose to break the memory bottleneck of the initial layers with \emph{patch-based inference} (Figure~\ref{fig:spatial_partial}).
Existing deep learning inference frameworks (\eg, TensorFlow Lite Micro~\cite{abadi2016tensorflow}, TinyEngine~\cite{lin2020mcunet}, microTVM~\cite{chen2018tvm}, \etc) use a \emph{layer-by-layer} execution. 
For each convolutional layer, the inference library first allocates the input and output activation buffer in SRAM, and releases the input buffer after the \emph{whole} layer computation is finished.
Such an implementation makes inference optimization easy (\eg, im2col,  tiling, \etc), but the SRAM has to hold the entire input and output activation for each layer, which is prohibitively large for the initial stage of the CNN.
Our patch-based inference runs the initial memory-intensive stage in a \emph{patch-by-patch} manner. For each time, we only run the model on a small spatial region (>10$\times$ smaller than the whole area), which effectively cuts down the peak memory usage. After this stage is finished, the rest of the network with a small peak memory is executed in a normal layer-by-layer manner (upper notations in Figure~\ref{fig:mbv2_mem}).


We show an example of two convolutional layers (with stride 1 and 2) in Figure~\ref{fig:spatial_partial}. For conventional per-layer computation, the first convolutional layer has large input and output activation size, leading to a high peak memory. With spatial partial computation, we allocate the buffer for the final output and compute its values \emph{patch-by-patch}. In this manner, we only need to store the activation from \emph{one patch} instead of the \emph{whole feature map}. Note that the first activation is the input image, which can be partially decoded from a compressed format like JPEG and does not require full storage.


\myparagraph{Computation overhead.}
The significant memory saving comes at the cost of computation overhead. To maintain the same output results as per-layer inference, the non-overlapping output patches correspond to overlapping patches in the input image (the shadow area in Figure~\ref{fig:spatial_partial}(b)). This is because convolutional filters with kernel size >1 contribute to increasing receptive fields. The bordering pixel on the output patches is dependent on the inputs from neighboring patches. Such repeated computation can increase the overall network computation by 10-17\% even under optimal hyper-parameter choice (Figure~\ref{fig:analytic_mem_flops}), which is undesirable for low-power edge devices. %



















\subsection{Reducing Computation Overhead by Redistributing the Receptive Field}

\begin{figure*}[t]
    \centering
     \includegraphics[width=0.9\textwidth]{mcunetv2/figures/mbv2_vs_mbv2rd.pdf}
    \caption{The redistributed MobileNetV2 (MbV2-RD) has reduced receptive field for the per-patch inference stage and increased receptive field for the per-layer stage. The two networks have the same level of performance, but MbV2-RD has a smaller overhead under patch-based inference. The mobile inverted block is denoted as \texttt{MB\{expansion ratio\} \{kernel size\}}. The dashed border means stride=2.
    }
    \label{fig:mbv2_vs_mbv2rd}
\end{figure*}

\input{mcunetv2/figure_text/tab_network_redistribute}

The computation overhead is related to the receptive field of the patch-based initial stage. Consider the output of the patch-based stage, the larger receptive field it has on the input image, the larger resolution for each patch, leading to a larger overlapping area and repeated computation (see Section~\ref{sec:ablation_study} for quantitative analysis). 
For MobileNetV2, if we only consider down-sampling, each input patch has a side length of $224/4=56$. But when considering the increased receptive field, each input patch has to use a shape of $75\times75$, leading to a large overlapping area. %


We propose to \emph{redistribute} the receptive field (RF) of the CNN to reduce computation overhead. The basic idea is: \emph{(1) reduce the receptive field of the patch-based initial stage;  (2) increase the receptive field of the later stage}. Reducing RF for the initial stage helps to reduce the size of each input patch and repeated computation. However, some tasks may have degraded performance if the overall RF is smaller (\eg, detecting large objects). Therefore, we further increase the RF of the later stage to compensate for the performance loss. 

We take MobileNetV2 as a study case and modify its architecture. The comparison is shown in Figure~\ref{fig:mbv2_vs_mbv2rd}. We used smaller kernels and fewer blocks in the per-patch inference stage, and increased the number of blocks in the later per-layer inference stage. The process needs manual tuning and varies case-by-case. We will later discuss how we \emph{automate} the process with NAS.
We compare the performance of the two architectures in Table~\ref{tab:network_redistribution}. 
Per-patch inference reduces the peak SRAM by 8$\times$ for all cases, but the original MobileNetV2 design has 42\% computation overhead for the patch-based stage and 10\% for the overall network. 
After redistributing the receptive field (``MbV2-RD''), we can reduce the input patch size from 75 to 63, while maintaining the same level of performance in image classification and object detection. After redistribution, the computation overhead is only 3\%, which is negligible considering the benefit in memory reduction.

\subsection{Joint Neural Architecture and Inference Scheduling Search}
\label{sec:joint_search}

Redistributing the receptive field allows us to enjoy the benefit of memory reduction at minimal computation/latency overhead, but the strategy varies case-by-case for different backbones. The reduced peak memory also allows larger freedom when designing the backbone architecture (\eg, using a larger input resolution). To explore such a large design space, we propose to jointly optimize the \emph{neural architecture} and the \emph{inference scheduling} in an automated manner.
Given a certain dataset and hardware constraints (SRAM limit, Flash limit, latency limit, \etc), our goal is to achieve the highest accuracy while satisfying all the constraints. We have the following knobs to optimize:

\myparagraph{Backbone optimization.} We follow~\cite{lin2020mcunet} to use a MnasNet-alike search space~\cite{tan2019mnasnet, cai2019proxylessnas} for NAS, so that we can have a fair comparison. The space includes different kernel sizes for each inverted residual block $k_{[~]}$ (3/5/7), different expansion ratios $e_{[~]}$ (3/4/6), and a different number of blocks for each stage $d_{[~]}$ (2/3/4). More recent search space designs like MobileNetV3~\cite{howard2019searching} have better accuracy-computation trade-off, but are hard to quantize due to Swish activation function~\cite{ramachandran2017searching}, making deployment on MCU difficult. 
As shown in~\cite{lin2020mcunet}, the search space configuration (\ie, the global width multiplier $w$ and input resolution $r$) is crucial to the final NAS performance. 
We argue that the best search space configuration is not only \emph{hardware-aware} but also \emph{task-aware}: for example, some tasks may prefer a higher resolution over a larger model size, and vice versa.
Therefore, we also put $r$ and $w$ into the search space. We further extend $w$ to support per-block width scaling $w_{[~]}$. Including $w_{[~]}$ (0.5/0.75/1.0) and $r$ (96-256)   expands the search space scalability, allowing us to fit different MCU models and tight resource budgets (ablation study provided in the supplementary).

\myparagraph{Inference scheduling optimization.} Given a model and hardware constraints, we will find the best inference scheduling. Our inference engine is developed based on TinyEngine~\cite{lin2020mcunet} to further patch-based inference. Apart from the optimization knobs in TinyEngine, 
we also need to determine the patches number $p$ and the number of blocks $n$ to perform patch-based inference, so that the inference satisfies the SRAM constraints. According to Section~\ref{sec:ablation_study}, a smaller $p$ and $n$ lead to a smaller computation overhead and faster inference. But it varies case-by-case, so we jointly optimize it with the architecture.

\myparagraph{Joint search.} 
We need to co-design the backbone optimization and inference scheduling. For example, given the same constraints, we can choose to use a smaller model that fits per-layer execution ($p=1$, no computation overhead), or a larger model and per-patch inference ($p>1$, with a small computation overhead). Therefore, we put both sides in the same loop and use evolutionary search to find the best set of $(k_{[~]}, e_{[~]}, d_{[~]}, w_{[~]}, r, p, n)$ satisfying constraints.
Specifically, we randomly sample neural networks from the super network search space; for each sampled network, we enumerate all the $p$ and $n$ choices (optimized together with other knobs in TinyEngine) and find the satisfying combinations. We then report the best $(p, n)$ pair with minimal computation/latency, and use the statistics to supervise architecture search. 
We provide the details and pseudo code in supplementary.%















==> mcunetv2/text/4_experiments.tex <==
\section{Experiments}


\myparagraph{Memory profiling.}
\label{sec:mem_profile}
The memory usage is dependent on the inference framework implementation~\cite{lin2020mcunet}. To ease the comparison, we study two profiling settings:

(1) We first study \emph{analytic profiling}, which is only related to the model architecture but not the inference framework. Following~\cite{chowdhery2019visual, saha2020rnnpool}, the memory required for a layer is the sum of input and output activation (since weights can be partially fetched from Flash); for networks with multi-branches (\eg, residual connection), we consider the sum of memory required for all branches at the same time (if the same input is shared by multiple branches, it will only be counted once). 



(2) We also study \emph{on-device profiling} to report the \emph{measured} SRAM and Flash usage when executing the deep model on MCU. The number is usually larger than the analytic results since we need to account for temporary buffers storing partial weights, Im2Col buffer, \etc. 

 
\myparagraph{Datasets.}
We analyze the advantage of our method on image classification datasets: ImageNet~\cite{deng2009imagenet} as the standard benchmark, and Visual Wake Words~\cite{chowdhery2019visual} to reflect TinyML applications. We further validate our method on object detection datasets: Pascal VOC~\cite{everingham2010pascal} and WIDER FACE~\cite{yang2016wider} to show our advantage: be able to fit larger resolution on the MCU.

\myparagraph{Training\&deployment.} We follow~\cite{lin2020mcunet} for super network training and evolutionary search, detailed in the supplementary. Models are quantized to \texttt{int8} for deployment. We extend TinyEngine~\cite{lin2020mcunet} to support patch-based inference, and benchmark the models on 3 MCU models with different hardware resources: STM32F412 (Cortex-M4, 256kB SRAM/1MB Flash), STM32F746 (Cortex-M7, 320kB SRAM/1MB Flash), STM32H743 (Cortex-M7, 512kB SRAM/2MB Flash). 



\subsection{Reducing Peak Memory of Existing Networks}

\input{mcunetv2/figure_text/fig_analytic_mem_flops}

We first analyze how patch-based inference can significantly reduce the peak memory for model inference, both in analytic profiling and on-device profiling.


\myparagraph{Analytic profiling.} We study several widely used deep network backbones designed for edge inference in Figure~\ref{fig:analytic_mem_flops}: MobileNetV2~\cite{sandler2018mobilenetv2} (MbV2), redistributed MobileNetV2 (MbV2-RD), Once-For-All CPU (OFA-CPU)~\cite{cai2020once}, MnasNet~\cite{tan2019mnasnet}, and FBNet-A~\cite{wu2019fbnet}.  All the networks use an input resolution of $224\times224$; for patch-based inference, we used $4\times4$ patches. The memory is profiled in \texttt{int8}.  Per-patch inference significantly reduces the peak memory by \textbf{3.7-8.0$\times$}, while only incurring \textbf{8-17\%} of computation overhead. 
For MobileNetV2, we can reduce the computation overhead from 10\% to 3\% by redistributing the receptive field without hurting accuracy (Table~\ref{tab:network_redistribution}).
The memory saving and computation reduction are related to the network architecture. Some models like MnasNet have a larger overhead since it uses large kernel sizes in the initial stage, which increases receptive fields. 
It shows the necessity to \emph{co-design} the network architecture with the inference engine.

\myparagraph{On-device measurement.} We further profile existing networks running on STM32F746 MCU. We measure the SRAM usage of the network with per-layer and per-patch ($2\times2$ or $3\times3$ patches) inference. Due to the memory limit of MCU (320kB SRAM, 1MB Flash), we have to scale down the width multiplier $w$ and input resolution $r$. As in Figure~\ref{fig:ondevice_mem_flops}, 
per-patch based inference reduces the measured peak SRAM by 4-6$\times$. 
Some models may have a large latency overhead, since the initial stage has worse hardware utilization. But with a proper architecture design (MbV2-RD), we can reduce the latency overhead to 4\%, 
which is negligible compared to the memory reduction benefit. 

\subsection{\method for Tiny Image Classification}
\label{sec:exp_image_cls}

With joint optimization of neural architecture and inference scheduling, \method significantly pushes the state-of-the-art results for MCU-based tiny image classification. 

\input{mcunetv2/figure_text/tab_mcu_imagenet}

\myparagraph{Pushing the ImageNet record on MCUs.} We compared \method with existing state-of-the-art solutions on ImageNet classification under two hardware settings: 256kB SRAM/1MB Flash and 512kB SRAM/2MB Flash. The former represents a widely used Cortex-M4 microcontroller; the latter corresponds to a  higher-end Cortex-M7. 
The goal is to achieve the highest ImageNet accuracy on resource-constrained MCUs (Table~\ref{tab:mcu_imagenet}). 
\method significantly improves the ImageNet accuracy of tiny deep learning on microcontrollers. Under 256kB SRAM/1MB Flash, \method outperforms the state-of-the-art method~\cite{lin2020mcunet} by 4.6\% at 18\% lower peak SRAM. Under 512kB SRAM/2MB Flash, \method achieves a new \emph{record} ImageNet accuracy of 71.8\% on commercial microcontrollers, which is 3.3\% compared to the best solution under the same quantization policy. 
Lower-bit (\texttt{int4}) or mixed-precision quantization can further improve the accuracy (marked in \textcolor{gray}{gray} in the table). We believe that we can further improve the accuracy of \method with a better quantization policy, which we leave to future work.


\input{mcunetv2/figure_text/fig_vww_curves}
\paragraph{Visual Wake Words under 32kB SRAM.} Visual wake word (VWW) reflects the low-energy application of tinyML. \method allows us to run a VWW model with a modest memory requirement. As in Figure~\ref{fig:vww_curves}, \method outperforms state-of-the-art method~\cite{lin2020mcunet} for both accuracy \vs peak memory and accuracy \vs latency trade-off. We perform neural architecture search under both \emph{per-layer} and \emph{per-patch} inference settings using the same search space and super network for ablation. Compared to per-layer inference, \method can achieve better accuracy using 4.0$\times$ smaller memory. Actually, it can achieve >90\% accuracy under 32kB SRAM requirement, allowing us to deploy the model on low-end MCUs like STM32F410 costing only \$1.6. For the latency-constrained setting, we jointly optimized the model architecture and inference scheduling, where a smaller patch number is used when possible.
Per-patch inference also expands the search space, giving us more freedom to find models with better accuracy \vs latency trade-off.  



\subsection{\method for Tiny Object Detection}
Object detection is sensitive to a smaller input resolution (Figure~\ref{fig:cls_det_degrade}). 
Current state-of-the-art~\cite{lin2020mcunet} cannot achieve a decent detection performance on MCUs due to the resolution bottleneck. \method breaks the memory bottleneck for detectors and improves the mAP by double digits. 

\myparagraph{MCU-based detection on Pascal VOC.}
\input{mcunetv2/figure_text/tab_mcu_det}
We show the object detection results on Pascal VOC trained with YOLOv3~\cite{redmon2018yolov3} on Table~\ref{tab:mcu_det}. We provide \method results for M4 MCU with 256kB SRAM and H7 MCU with 512kB SRAM. On H7 MCU, \method{-H7} improves the mAP by 16.7\% compared to the state-of-the-art method MCUNet~\cite{lin2020mcunet}. It can also scale down to fit a cheaper commodity Cortex-M4 MCU with only 256kB SRAM, while still improving the mAP by 13.2\% at 1.9$\times$ smaller peak SRAM.
Note that \method{-M4} shares a similar computation with MCUNet  (172M \vs 168M) but a much better mAP. This is because the expanded search space from patch-based inference allows us to choose a better configuration of larger input resolution and smaller models. 


\myparagraph{Memory-efficient face detection.}
\input{mcunetv2/figure_text/tab_wider_face}
We benchmarked \method for memory-efficient face detection on WIDER FACE~\cite{yang2016wider} dataset in Table~\ref{tab:wider_face}. We report the analytic memory usage of the detector backbone in \texttt{fp32} following~\cite{saha2020rnnpool}. We train our methods with  S3FD face detector~\cite{zhang2017s3fd} following~\cite{saha2020rnnpool} for a fair comparison. 
We also report mAP on samples with $\leq$ 3 faces, which is a more realistic setting for tiny devices.  
\method outperforms existing solutions under different scales.  \method{-L} achieves comparable performance at 3.4$\times$ smaller peak memory compared to RNNPool-Face-C~\cite{lin2020mcunet} and 9.9$\times$ smaller peak memory compared to LFFD~\cite{he2019lffd}. The computation is also 1.6$\times$ and 8.4$\times$ smaller.
\method{-S} consistently outperforms RNNPool-Face-A~\cite{saha2020rnnpool} and EagleEye~\cite{zhao2019real} at 1.8$\times$ smaller peak memory. 



\subsection{Analysis}
\label{sec:ablation_study}
\input{mcunetv2/figure_text/fig_granularity_study}
\myparagraph{Hyper-parameters for patch-based inference.}
We study the hyper-parameters used for patch-based inference: the number of blocks to be executed under patch-based inference $n$; the number of patches to split the input image $p$ (splitting the image into $p\times p$ overlapping patches). We analyze MobileNetV2~\cite{sandler2018mobilenetv2} in Figure~\ref{fig:granularity_study}(a), with a larger $n$, the patch size increases due to the growing receptive field. The peak memory first goes down since the output feature map is smaller then goes up due to larger receptive field overhead. $n=5$ is optimal.
For a larger $p$ (given $n$=5), each patch is smaller, which helps to reduce the peak memory. However, it also leads to more computation overhead due to more spatial overlapping (Figure~\ref{fig:granularity_study}(b)). Receptive field redistribution can reduce the overhead significantly (MbV2-RD). The optimal design is $n^*=5, p^*=4$ to reach the minimum peak memory with the smallest overhead.
The choice of $p$ and $n$ varies for different networks. Therefore, we use an automated method to jointly optimize with neural architecture (Section~\ref{sec:joint_search}).

\myparagraph{Comparison to other solutions. }

\input{mcunetv2/figure_text/tab_compare_other_method}

We also compare \method with other methods that reduce inference peak memory. The comparison on MobileNetV2~\cite{sandler2018mobilenetv2} is shown in Table~\ref{tab:compare_methods}. A straightforward way is to split the input image into \emph{non-overlapping} patches (``Non-overlap'') for the first several blocks as done in~\cite{dosovitskiy2020image}. Such a practice does not incur extra computation, but it breaks the feature propagation between patches and the translational invariance of CNNs. It achieves lower image classification accuracy and significantly degraded object detection mAP (on Pascal VOC) due to the lack of cross-patch communication (a similar phenomenon is observed in~\cite{liu2021swin}). For MobileNetV2 with RNNPool~\cite{saha2020rnnpool}, it can reduce the peak memory but leads to inferior ImageNet accuracy and object detection mAP. Its training time is also 3.2$\times$ longer\footnote{measured with official PyTorch code (MIT License) 
using a batch size of 64 on NVIDIA Titan RTX.
} due to the complicated data path and the RNN module. On the other hand, \method acts exactly the same as a normal network during training (per-layer forward/backward), while also matching the image classification and objection detection performance.
\method can further improve the results with joint neural architecture and inference scheduling search (Section~\ref{sec:exp_image_cls}). 


\myparagraph{Dissecting \method architecture.}
\begin{figure*}[t]
    \centering
     \includegraphics[width=0.8\textwidth]{mcunetv2/figures/example_arch.pdf}
    \caption{An \method architecture on VWW. The color represents the kernel size; the height of each block represents the expansion ratio. The name is \texttt{MB\{expansion ratio\} \{kernel size\}x\{kernel size\}}. Blocks with dashed borders have stride=2. \texttt{\{\}x\{\}} in the bottom denotes the feature map resolution.
    }
    \label{fig:example_arch}
\end{figure*}


We visualize one of the \method model architecture on the VWW~\cite{chowdhery2019visual} dataset in Figure~\ref{fig:example_arch}. We can find the following patterns:

\begin{itemize}
    \item The kernel size in the per-patch inference stage is small ($1\times1$ and $3\times3$) to reduce the receptive field and spatial overlapping, thus reducing computation overhead.
    \item The expansion ratio of the middle stage (early in per-layer stage) is small to further reduce the peak memory; while the expansion ratio for the later stage is large to increase performance.
    \item Large expansion ratios and large kernel sizes usually do not appear together to reduce the computational cost and latency: if the expansion ratio is large (like 6), the kernel size is small ($3\times3$ or $5\times5$); if the kernel size is large ($7\times7$), the expansion ratio is small (3 or 4).
    \item The input resolution is larger on resolution-sensitive datasets like VWW compared to MCUNet~\cite{lin2020mcunet}, since per-layer inference cannot fit a large input resolution.
\end{itemize}

Notice that all the patterns are automatically discovered by the joint neural architecture and inference scheduling search algorithm, without human expertise.

















 


==> mcunetv2/text/5_conclusion.tex <==
\section{Conclusion}
In this paper, we propose patch-based inference to reduce the memory usage for tiny deep learning by up to 8$\times$, which greatly expands the design space and unlocks powerful vision applications on IoT devices. We jointly optimize the neural architecture and inference scheduling to develop \method. 
\method significantly improves the object detection performance on microcontrollers by 16.9\% and achieves a record ImageNet accuracy (71.8\%). For the VWW dataset, \method can achieve >90\% accuracy under only 32kB SRAM, 4$\times$ smaller than existing work. Our study largely addresses the memory bottleneck in tinyML and paves the way for vision applications beyond classification.


\section*{Acknowledgments}
We thank MIT-IBM Watson AI Lab, Samsung, Woodside Energy, and NSF CAREER Award \#1943349 for supporting this research.

==> mcunetv3/figure_text/fig_sparse_update.tex <==

\begin{figure*}[t]
    \centering
     \includegraphics[width=0.95\textwidth]{mcunetv3/figures/sparse_update.pdf}
     \vspace{-5pt}
    \caption{Different update paradigms of two linear layers in a deep neural network.
    }
    \label{fig:sparse_update}
\end{figure*}





==> mcunetv3/figure_text/fig_visualize_scheme.tex <==

\begin{figure*}[t]
    \centering
     \includegraphics[width=\textwidth]{mcunetv3/figures/update_scheme_addfc.pdf}
     \vspace{-15pt}
    \caption{\textbf{(a)} The weight and activation memory cost of updating \emph{each} layer of MCUNet (analytic). We find that the activation cost is high for the starting layers; the weight cost is high for the later layers; the overall memory cost is low for the middle layers. \textbf{(b)} Dissecting the sparse update scheme: we update the biases of the last 22 layers due to its low activation cost. For weight update, we update some middle layers due to its low memory cost, and update partial channels of the two later layers since they are important for accuracy (Figure~\ref{fig:sensitivity_curve}).} 
    \label{fig:update_scheme}
    % \vspace{-15pt}
\end{figure*}

==> mcunetv3/figure_text/tab_single_vs_batch.tex <==


\definecolor{this_gray}{rgb}{0.8,0.8,0.8}
\begin{table}[H]
    \caption{Momentum helps transfer learning with batch size 128, but not with batch size 1; without momentum, we can use the normal-batch training results as an approximation for single-batch training.
    Results obtained by updating the last two blocks of MCUNet~\cite{lin2020mcunet} with SGD+QARS.
    }
    \label{tab:single_batch}
    \centering
    \small{
     \begin{tabular}{llcccccccc}
    \toprule
 \multirow{2}{*}{Batch size} & \multirow{2}{*}{Momentum} & \multirow{2}{*}{Mem Cost} & \multicolumn{5}{c}{Accuracy (\%)} & \multirow{2}{*}{\shortstack{Avg\\Acc.}} \\ \cmidrule(lr){4-8}
 & & & Cars &  CUB & Flowers & Pets & VWW \\
\midrule
 \multirow{2}{*}{128 \textcolor{this_gray}{(GPU simulate)}} & 0.9 & 2$\times$ & 55.2 & 57.8 & 89.1 & 80.9  & 89.3 & 74.4 \\ 
 & 0 &  1$\times$ & 47.8 & 57.2 & 87.3 & 80.8 & 88.8&  72.4  \\ \midrule 
\multirow{2}{*}{1 \textcolor{this_gray}{(tinyML)} } & 0.9 &  2$\times$& 47.8 &  54.8 & 88.5 & 80.5 & 86.2  & 71.5 \\ 
& 0 &   1$\times$ &51.1 &  56.2 & 88.7 & 79.3 & 86.0 &  72.3 \\ 
    \bottomrule
     \end{tabular}
     }
\end{table}


==> mcunetv3/main.tex <==
\def\engine{Tiny Training Engine\xspace}
\def\engineshort{TTE\xspace}

\definecolor{fig5gray}{rgb}{0.80, 0.85, 0.89}
\definecolor{fig5red}{rgb}{1.00, 0.59, 0.55}
\definecolor{fig5yellow}{rgb}{1.00, 0.68, 0.00}

\input{mcunetv3/text/0_abstract}
\input{mcunetv3/text/1_introduction}
\input{mcunetv3/text/3_approach}
\input{mcunetv3/text/4_experiments}
\input{mcunetv3/text/2_related_work}
\input{mcunetv3/text/5_conclusion}




==> mcunetv3/text/0_abstract.tex <==
\begin{abstract}

On-device training enables the model to adapt to new data collected from the sensors by fine-tuning a pre-trained model. However, the training memory consumption is prohibitive for IoT devices that have tiny memory resources.
We propose an algorithm-system co-design framework
to make on-device training possible with only \emph{256KB} of memory. On-device training faces two unique challenges: (1) the quantized graphs of neural networks are hard to optimize due to mixed bit-precision and the lack of normalization; (2) the limited hardware resource (memory and computation) does not allow full backward computation.
To cope with the optimization difficulty,
we propose \textit{\textbf{Quantization-Aware Scaling}}  to calibrate the gradient scales and stabilize quantized training.
To reduce the memory footprint, we propose \textit{\textbf{Sparse Update}} to skip the gradient computation of less important layers and sub-tensors.
The algorithm innovation is implemented by a lightweight training system, \textit{\textbf{\engine}}, which prunes the backward computation graph to support sparse updates and offload the runtime auto-differentiation to compile time.
Our framework is the \emph{first} practical solution for on-device transfer learning of visual recognition on tiny IoT devices (\eg, a microcontroller with only 256KB SRAM), using less than 1/100 of the memory of existing frameworks while matching the accuracy of cloud training+edge deployment for the tinyML application VWW~\cite{chowdhery2019visual}. Our study enables IoT devices to not only perform inference but also continuously adapt to new data for on-device lifelong learning. %





\end{abstract}





==> mcunetv3/text/1_introduction.tex <==
\vspace{-5pt}
\section{Introduction}

On-device training allows us to \emph{adapt} the pre-trained model to newly collected sensory data \emph{after} deployment.  By training and adapting \emph{locally} on the edge, the model can learn to continuously improve its predictions and perform lifelong learning and user customization. By bringing training closer to the sensors, it also helps to protect user privacy when handling sensitive data (\eg, healthcare). 

However, on-device training on tiny edge devices is extremely challenging and fundamentally different from cloud training. Tiny IoT devices (\eg, microcontrollers) typically have a limited SRAM size like 256KB. Such a small memory budget is hardly enough for the \emph{inference} of deep learning models~\cite{lin2020mcunet, lin2021mcunetv2, banbury2021micronets, burrello2021dory, liberis2020mu, fedorov2019sparse, liberis2019neural, rusci2019memory}, let alone the \emph{training}, which requires extra computation for the backward and extra memory for intermediate activation~\cite{chen2016training}. On the other hand, modern deep training frameworks (\eg, PyTorch~\cite{pytorch2019}, TensorFlow~\cite{tensorflow2015}) are usually designed for cloud servers and require a large memory footprint (>300MB) even when training a small model (\eg, MobileNetV2-w0.35~\cite{sandler2018mobilenetv2}) with batch size 1. 
The huge gap (>1000$\times$) makes it impossible to run on tiny IoT devices. Furthermore, devices like microcontrollers are bare-metal and do not have an operational system and the runtime support needed by existing training frameworks. Therefore, we need to jointly design the \emph{algorithm} and the \emph{system} to enable tiny on-device training.


Deep learning training systems like PyTorch~\cite{pytorch2019}, TensorFlow~\cite{tensorflow2015}, JAX~\cite{jax2018github}, MXNet~\cite{chen2015mxnet}, \etc 
do not consider the tight resources on edge devices. Edge deep learning inference frameworks like TVM~\cite{chen2018tvm}, TF-Lite~\cite{tflite}, NCNN~\cite{tensorRT}, \etc provide a slim runtime, but lack the support for back-propagation. There are low-cost efficient transfer learning algorithms like training only the final classifier layer, bias-only update~\cite{cai2020tinytl}, \etc. However, existing training system can not realize the theoretical saving into measured saving. The downstream accuracy of such update schemes is also low (Figure~\ref{fig:acc_vs_mem}). 

\input{mcunetv3/figure_text/fig_teaser_mem_compare}

In this paper, we aim to bridge the gap and enable tiny on-device training with algorithm-system co-design. We investigate tiny on-device training and find two unique challenges: (1) the model is quantized on edge devices. A \emph{real} quantized graph is difficult to optimize due to mixed-precision tensors and the lack of Batch Normalization layers~\cite{ioffe2015batch}; (2) the limited hardware resource (memory and computation) of tiny hardware does not allow full back-propagation, whose memory usage can easily exceed the SRAM of microcontrollers by more than an order of magnitude. Only updating the last layer leads to poor accuracy (Figure~\ref{fig:acc_vs_mem}). To cope with the optimization difficulty, we propose \textit{\textbf{Quantization-Aware Scaling (QAS)}} to automatically scale the gradient of tensors with different bit-precisions, which effectively stabilizes the training and matches the accuracy of the floating-point counterpart (Section~\ref{sec:opt_mixed_prec}). QAS is hyper-parameter free and no tuning is required. To reduce the memory footprint of the full backward computation, we propose \textit{\textbf{Sparse Update}} to skip the gradient computation of less important layers and sub-tensors. We developed an automated method based on contribution analysis to find the best update scheme under different memory budgets (Section~\ref{sec:method:sparse_update}). Finally, we propose a lightweight training system, \textit{\textbf{\engine (\engineshort)}} , to assist with the algorithm innovation (Section~\ref{sec:engine}). \engineshort is based on code generation; it offloads the auto-differentiation to the compile-time to greatly cut down the runtime overhead. It also supports advanced graph optimization like graph pruning and reordering to support sparse updates, achieving measured memory saving and speedup.

Our framework is the \textbf{first} solution to actually enable tiny on-device training of convolutional neural networks under \textbf{256KB} memory budget. \textbf{(1)} Our solution enables the parameter update not only for the \emph{classifier} but also for the \emph{backbone}, which provides a \emph{high transfer learning accuracy} (Figure~\ref{fig:acc_vs_mem}). For tinyML application VWW~\cite{chowdhery2019visual}, our on-device finetuned model matches the accuracy of cloud training+edge deployment, and surpasses the common requirement of tinyML (MLPerf Tiny~\cite{banbury2020benchmarking}) by 9\%.
\textbf{(2)} Our system-algorithm co-design scheme effectively \emph{reduces the memory footprint}. As shown in Figure~\ref{fig:teaser}, the proposed techniques greatly reduce the memory usage by more than 1000$\times$ compared to cloud training frameworks, and more than 100$\times$ compared to the best edge training framework we can find (MNN~\cite{jiang2020mnn}). 
\textbf{(3)} Our framework also greatly \emph{accelerates training}, reducing the per-iteration time by more than 20$\times$ compared to dense update and vanilla system design (Figure~\ref{fig:latency_peakmem_comparison}), leading to significant energy saving and promoting practical usage.
\textbf{(4)} We deployed our training system to a microcontroller STM32F746 to demonstrate the feasibility. Our study suggests that tiny IoT devices can not only perform inference but also adapt to new data and enjoy lifelong learning capabilities. %























==> mcunetv3/text/2_related_work.tex <==
\vspace{-5pt}
\section{Related Work}

\myparagraph{Efficient transfer learning.}
There are several ways to reduce the transfer learning cost compared to fine-tuning the full model~\cite{kornblith2019better,cui2018large, kolesnikov2020big}. 
The most straightforward way is to only update the classifier layer~\cite{chatfield2014return,donahue2014decaf,gan2015devnet,sharif2014cnn}, but the accuracy is low when the domain shift is large~\cite{cai2020tinytl}. 
Later studies investigate other tuning methods including updating biases~\cite{cai2020tinytl, zaken21bitfit}, updating normalization layer parameters~\cite{mudrakarta2019k,frankle2020training}, updating small parallel branches~\cite{cai2020tinytl, hu2021lora}, \etc. 
These methods only reduce the trainable parameter number but lack the study on system co-design to achieve real memory savings. Most of them do not fit tinyML settings (cannot handle quantized graph and lack of BatchNorm~\cite{ioffe2015batch}).

\myparagraph{Systems for deep learning.}
The success of deep learning is built on top of popular training frameworks such as  PyTorch~\cite{pytorch2019}, TensorFlow~\cite{abadi2016tensorflow}, MXNet~\cite{chen2015mxnet}, JAX~\cite{jax2018github}, \etc. These systems usually depend on a host language (\eg Python) and various runtimes, which brings 
significant overhead (>300MB) and does not fit tiny edge devices.
Inference libraries like TVM~\cite{chen2018tvm}, TF-Lite~\cite{tflite}, MNN~\cite{jiang2020mnn}, NCNN~\cite{ncnn}, TensorRT~\cite{tensorRT}, and OpenVino~\cite{vaswani2017attention} provide lightweight runtime environments but do not support training (only MNN has preliminary support for full model training). None of the existing frameworks can fit tiny IoT devices with tight memory constraints. 


\myparagraph{Tiny deep learning on microcontrollers.}
Tiny deep learning on microcontrollers is challenging. 
Existing work explores model compression (pruning~\cite{han2016deep, he2018amc, lin2017runtime, he2017channel, liu2017learning, yu2017scalpel, liberis2021differentiable}, quantization~\cite{han2016deep, rastegari2016xnor, wang2019haq, choi2018pact, rusci2019memory, langroudi2021tent, lin2020mcunet, jacob2018quantization}) and neural architecture search~\cite{zoph2017neural, zoph2018learning, tan2019mnasnet, lin2020mcunet, banbury2021micronets, liberis2020mu, fedorov2019sparse, lyu2021resource, lin2020mcunet, lin2021mcunetv2} to reduce the required resource of deep learning models. There are several deep learning systems for tinyML (TF-Micro~\cite{abadi2016tensorflow}, CMSIS-NN~\cite{lai2018cmsis}, TinyEngine~\cite{lin2020mcunet}, MicroTVM~\cite{chen2018tvm}, CMix-NN~\cite{capotondi2020cmix}, \etc). However, the above algorithms and systems are only for inference but not training. 
There are several preliminary attempts to explore training on microcontrollers~\cite{ren2021tinyol, grau2021device, sudharsan2021train, sudharsan2021globe2train}. However, due to the lack of efficient algorithm and system support, they are only able to tune one layer or a very small model, while our work supports the tuning of modern CNNs for real-life applications. 


















==> mcunetv3/text/3_approach.tex <==
\vspace{-5pt}
\section{Approach}

Neural networks usually need to be quantized to fit the limited memory of edge devices~\cite{lin2020mcunet, jacob2018quantization}. 
For a \texttt{fp32} linear layer
$\mathbf{y}_{\texttt{fp32}} = \mathbf{W}_{\texttt{fp32}}\mathbf{x}_{\texttt{fp32}} + \mathbf{b}_{\texttt{fp32}}$, the \texttt{int8} quantized counterpart is:
\begin{equation}  \label{eq:quantize_forward}
\mathbf{\bar{y}}_{\texttt{int8}} = \texttt{cast2int8}[s_{\texttt{fp32}} \cdot(\mathbf{\bar{W}}_{\texttt{int8}}\mathbf{\bar{x}}_{\texttt{int8}} + \mathbf{\bar{b}}_{\texttt{int32}})],
\end{equation}\useshortskip
where $\bar{\cdot}$ denotes the tensor being quantized to fixed-point numbers, and $s$ is a floating-point scaling factor to project the results back into \texttt{int8} range. 
We compute the gradient update for the weights as:
$\mathbf{\bar{W}^\prime}_{\texttt{int8}} = \texttt{cast2int8}(\mathbf{\bar{W}_{\texttt{int8}}} - \alpha\cdot \mathbf{G_\mathbf{\bar{W}}})$,
where $\alpha$ is the learning rate, and $\mathbf{G_\mathbf{\bar{W}}}$ is the gradient of the weights. After applying the gradient update, we round the weights back to 8-bit integers.

\subsection{Optimizing Real Quantized Graphs}
\label{sec:opt_mixed_prec}
Unlike fine-tuning floating-point model on the cloud, training with \textit{a real} quantized graph\footnote{Note that this is contrary to the \textit{fake} quantization 
graph widely used in quantization-aware training~\cite{jacob2018quantization}. 
Please refer to Section~\ref{sec:real_vs_fake_quantize} for details. 
} is difficult: the quantized graph has tensors of different bit-precisions (\texttt{int8}, \texttt{int32}, \texttt{fp32}, shown in Equation~\ref{eq:quantize_forward})
and lacks Batch Normalization~\cite{ioffe2015batch} layers (fused), leading to unstable gradient update.


\input{mcunetv3/figure_text/fig_per_layer_wg_ratio}

\myparagraph{Gradient scale mismatch.}
When optimizing a quantized graph, the accuracy is lower compared to the floating-point counterpart. We hypothesize that the quantization process distorts the gradient update. 
To verify the idea, we plot the ratio between weight norm and gradient norm (\ie, $\lVert \mathbf{W}\rVert/\lVert\mathbf{G}\rVert$) for each tensor at the beginning of the training on the CIFAR dataset~\cite{krizhevsky2009learning} in Figure~\ref{fig:per_layer_wg_rate}. The ratio curve is very different after quantization: (1) the ratio is much larger (could be addressed by adjusting the learning rate); (2) the ratio has a different pattern after quantization. Take the highlighted area (red box) as an example, the quantized ratios have a zigzag pattern, differing from the floating-point curve.
If we use a fixed learning rate for all the tensors, then the update speed of each tensor would be very different compared to the floating-point case, leading to inferior accuracy. We empirically find that adaptive-learning rate optimizers like Adam~\cite{kingma2014adam} cannot fully address the issue (Section~\ref{sec:exp_qas}).




\myparagraph{Quantization-aware scaling (QAS).} 
To address the problem, we propose a hyper-parameter-free learning rate scaling rule, QAS.
Consider a 2D weight matrix of a linear layer $\mathbf{W}\in \mathds{R}^{c_1\times c_2}$, where $c_1, c_2$ are the input and output channel. To perform per-tensor quantization\footnote{For simplicity. We actually used per-channel quantization~\cite{jacob2018quantization} and the scaling factor is a vector of size $c_2$.}, we compute a scaling rate $s_\mathbf{W}\in\mathds{R}$, such that $\mathbf{\bar{W}}$'s largest magnitude is $2^7-1=127$: %
\begin{equation}
\mathbf{W} = s_\mathbf{W}\cdot(\mathbf{W} / s_\mathbf{W}) \stackrel{\text{quantize}}{\approx} s_\mathbf{W} \cdot \mathbf{\bar{W}}, \quad \mathbf{G_{\bar{W}}} \approx s_\mathbf{W}\cdot \mathbf{G_W},
\end{equation}
The process (roughly) preserves the mathematical functionality during the forward (Equation~\ref{eq:quantize_forward}), but it distorts the magnitude ratio between the weight and its corresponding gradient:
\begin{equation}\label{eq:wg_ratio}
  \lVert \mathbf{\bar{W}} \rVert / \lVert \mathbf{G_{\bar{W}}} \rVert \approx \lVert \mathbf{W}  /s_\mathbf{W} \rVert / \lVert s_\mathbf{W}\cdot \mathbf{G_W}\rVert = s_\mathbf{W}^{-2} \cdot \lVert\mathbf{W}\rVert / \lVert\mathbf{G}\rVert.
\end{equation}
We find that the weight and gradient ratios are off by  $s_\mathbf{W}^{-2}$, leading to the distorted pattern in Figure~\ref{fig:per_layer_wg_rate}: (1) the scaling factor is far smaller than 1, making the weight-gradient ratio much larger; (2) weights and biases have different data type (\texttt{int8} \vs \texttt{int32}) and thus have scaling factors of very different magnitude, leading to the zigzag pattern.
To solve the issue, we propose Quantization-Aware Scaling (QAS) by compensating the gradient of the quantized graph according to Equation~\ref{eq:wg_ratio}:
\begin{equation} \label{eq:qas}
    \mathbf{\Tilde{G}_{\bar{W}}} = \mathbf{G_{\bar{W}}} \cdot s_\mathbf{W}^{-2}, \quad 
    \mathbf{\Tilde{G}_{\bar{b}}} = \mathbf{G_{\bar{b}}} \cdot s_\mathbf{W}^{-2} \cdot s_{\mathbf{x}}^{-2} = \mathbf{G_{\bar{b}}} \cdot s^{-2}
\end{equation}
where $s_{\mathbf{X}}^{-2}$ is the scaling factor for quantizing input $\mathbf{x}$ (a scalar following~\cite{jacob2018quantization}, note that $s=s_\mathbf{W} \cdot s_{\mathbf{x}}$ in Equation~\ref{eq:quantize_forward}).
We plot the $\lVert \mathbf{W}\rVert/\lVert\mathbf{G}\rVert$ curve with QAS in Figure~\ref{fig:per_layer_wg_rate} (int8+scale). After scaling, the gradient ratios  match the floating-point counterpart. It also improves transfer learning accuracy (Table~\ref{tab:optimizer_study}), matching the accuracy of the floating-point counterpart without incurring memory overhead.   









\subsection{Memory-Efficient Sparse Update} 
\label{sec:method:sparse_update}
\input{mcunetv3/figure_text/fig_sparse_update}
Though QAS makes optimizing a quantized model possible, 
updating the whole model (or even the last several blocks) requires a large amount of memory, which is not affordable for the tinyML setting.  We propose to sparsely update the layers and the tensors.



\myparagraph{Sparse layer/tensor update.}
Pruning techniques prove to be quite successful for achieving sparsity and reducing model size~\cite{han2016deep, he2018amc, lin2017runtime, he2017channel, liu2017learning, liu2019metapruning}. 
Instead of pruning \emph{weights} for inference, we "prune" the \emph{gradient} during backpropagation, and update the model sparsely. Given a tight memory budget, we skip the update of the \emph{less important} parameters to reduce memory usage and computation cost. 
We consider updating a linear layer $\mathbf{y}=\mathbf{W}\mathbf{x}+\mathbf{b}$ (similar analysis applies to convolutions).
Given the output gradient $\mathbf{G_y}$ from the later layer, we can compute the gradient update by $\mathbf{G_W}=f_1(\mathbf{G_y}, \mathbf{x})$ and $\mathbf{G_b}=f_2(\mathbf{G_y})$. Notice that updating the biases does not require saving the intermediate activation $\mathbf{x}$, leading to a lighter memory footprint~\cite{cai2020tinytl}\footnote{If we update many layers, the intermediate activation could consume a large memory~\cite{chen2016training}.}; while updating the weights is more memory-intensive but also more expressive. For hardware like microcontrollers, we also need an extra copy for the updated parameters since the original ones are stored in read-only FLASH~\cite{lin2020mcunet}.
Given the different natures of updating rules, we consider the sparse update rule in three aspects (Figure~\ref{fig:sparse_update}):
(1) \emph{Bias update}: how many layers should we backpropagate to and update the biases (bias update is cheap, we always update the biases if we have backpropagated to a layer).
(2) \emph{Sparse layer update}: select a subset of layers to update the corresponding weights.
(3) \emph{Sparse tensor update}: we further allow updating a subset of weight channels to reduce the cost. %

However, finding the right sparse update scheme under a memory budget is challenging due to the large combinational space. For MCUNet~\cite{lin2020mcunet} model with 43 convolutional layers and weight update ratios from \{0, 1/8, 1/4, 1/2, 1\},
the combination is about $10^{30}$, making exhaustive search impossible.





\input{mcunetv3/figure_text/fig_sensitivity_curve}

\myparagraph{Automated selection with contribution analysis.} 
We propose to automatically derive the sparse update scheme by \emph{contribution analysis}. We find the contribution of each parameter (weight/bias) to the downstream accuracy.
Given a convolutional neural network with $l$ layers, we measure the accuracy improvement from (1) biases: the improvement of updating \emph{last} $k$ biases $\textbf{b}_{l}, \textbf{b}_{l-1},..., \textbf{b}_{l-k+1}$ (bias-only update) compared to only updating the classifier, defined as $\Delta\text{acc}_{\textbf{b}[:k]}$; (2) weights: the improvement of updating the weight of one extra layer $\textbf{W}_i$ (with a channel update ratio $r$) compared to bias-only update, defined as $\Delta\text{acc}_{\textbf{W}i, r}$. An example of the contribution analysis can be found in Figure~\ref{fig:sensitivity_curve} (MCUNet on Cars~\cite{krause20133d} dataset; please find more results in appendix Section~\ref{sec:more_contribution}).
After we find $\Delta\text{acc}_{\textbf{b}[:k]}$ and $\Delta\text{acc}_{\textbf{W}i}$ ($1\leq k, i\leq l$), we solve an optimization problem to find:
\begin{equation}
    k^*, \mathbf{i}^*, \mathbf{r}^* = \max_{k, \mathbf{i}, \mathbf{r}} (\Delta\text{acc}_{\textbf{b}[:k]} + \sum_{i\in\mathbf{i}, r\in\mathbf{r}} \Delta\text{acc}_{\textbf{W}i, r}) \quad
    \text{s.t. Memory}(k, \mathbf{i}, \mathbf{r}) \leq \text{constraint},
\end{equation}
where $\mathbf{i}$ is a collection of layer indices whose weights are updated, and $\mathbf{r}$ is the corresponding update ratios (1/8, 1/4, 1/2, 1). Intuitively, by solving this optimization problem, we find the combination of (\#layers for bias update, the subset of weights to update), such that the total contribution are maximized  while the memory overhead does not exceed the constraint. The problem can be efficiently solved with evolutionary search (see Section~\ref{sec:evo_vs_random}). 
Here we assume that the accuracy contribution of each tensor ($\Delta\text{acc}$) can be summed up. Such approximation is quite effective (Figure~\ref{fig:sensitivity_curve}(c)).

\subsection{\engine (\engineshort)}
\label{sec:engine}
\input{mcunetv3/figure_text/fig_compiler_stack}

The theoretical saving from real quantized training and sparse update does not translate to measured memory saving in existing deep learning frameworks, due to the redundant runtime and the lack of graph pruning.
We co-designed an efficient training system, \engine (\engineshort), to transform the above algorithms into slim binary codes (Figure~\ref{fig:compiler_stack}). %

\myparagraph{Compile-time differentiation and code generation.}
\engineshort offloads the auto-differentiation from the runtime to the compile-time, generating a static backward graph which can be pruned and optimized (see below) to reduce the memory and computation. \engineshort is based on code generation: it compiles the optimized graphs to executable binaries on the target hardware, which minimizes the runtime library size and removes the need for host languages like Python (typically uses Megabytes of memory).

\myparagraph{Backward graph pruning for sparse update.}
We prune the redundant nodes  in the backward graph before compiling it to binary codes.
For sparse layer update, we prune away the gradient nodes of the frozen weights, only keeping the nodes for bias update. Afterwards, we traverse the graph to find unused intermediate nodes due to pruning (\eg, saved input activation) and apply dead-code elimination (DCE) to remove the redundancy. 
For sparse tensor update, we introduce a \emph{sub-operator slicing} mechanism to split a layer's weights into trainable and frozen parts; the backward graph of the frozen subset is removed. 
Our compiler translates the sparse update algorithm into measured memory saving, reducing the training memory by 7-18$\times$ without losing accuracy (Figure~\ref{fig:latency_peakmem_comparison}(a)).

\input{mcunetv3/figure_text/fig_mem_footprint}
\myparagraph{Operator reordering.}
The execution order of different operations affects the life cycle of tensors and the overall memory footprint. This has been well-studied for inference~\cite{ahn2020ordering, liberis2019neural} but not for training due to the extra complexity.
Traditional training frameworks usually derive the gradients of all the trainable parameters before applying the update. Such a practice leads to a significant memory waste for storing the gradients. By reordering operators, we can immediately apply the gradient update to a specific tensor (in-place update) before back-propagating to earlier layers, so that the gradient can be released. As such, we trace the dependency of all tensors (weights, gradients, activation) and reorder the operators, so that some operators can be fused to reduce memory footprint (by 1.6-3.4$\times$, Figure~\ref{fig:latency_peakmem_comparison}(a)). We provide an example in Figure~\ref{fig:mem_footprint} to reflect the memory saving from reordering. 



































    


==> mcunetv3/text/4_experiments.tex <==
\vspace{-5pt}
\section{Experiments}

\subsection{Setups}
\label{sec:exp_setup}
\myparagraph{Training.}
We used three popular tinyML models in our experiments: MobileNetV2~\cite{sandler2018mobilenetv2} (width multiplier 0.35, backbone 17M MACs, 0.25M Param), 
ProxylessNAS~\cite{cai2019proxylessnas} (width multiplier 0.3, backbone 19M MACs, 0.33M Param), 
MCUNet~\cite{lin2020mcunet} (the 5FPS ImageNet model, backbone 23M MACs, 0.48M Param).
We pre-trained the models on ImageNet~\cite{deng2009imagenet} and perform post-training quantization~\cite{jacob2018quantization}. The quantized models are fine-tuned on downstream datasets to evaluate the transfer learning capacity. 
We perform the training and memory/latency measurement on a microcontroller STM32F746 (320KB SRAM, 1MB Flash) using a single batch size. To faster obtain the accuracy statistics on multiple downstream datasets, we simulate the training results on GPUs, and we verified that the simulation obtains the same level of accuracy compared to training on microcontrollers.
Please refer to the the appendix (Section~\ref{sec:training_details}) for detailed training hyper-parameters.
We also provide a \emph{video demo} of deploying our training system on microcontroller in the appendix (Section~\ref{sec:video_demo}).



\myparagraph{Datasets.}
We measure the transfer learning accuracy on multiple downstream datasets and report the average accuracy~\cite{kolesnikov2020big}. We follow~\cite{cai2020tinytl} to use a set of vision datasets including Cars~\cite{krause20133d}, CIFAR-10~\cite{krizhevsky2009learning}, CIFAR-100~\cite{krizhevsky2009learning}, CUB~\cite{cub}, Flowers~\cite{nilsback2008automated}, Food~\cite{bossard2014food}, and Pets~\cite{parkhi2012cats}\footnote{Pets uses \href{https://creativecommons.org/licenses/by-sa/4.0/}{CC BY-SA 4.0} license; Cars and ImageNet use \href{https://image-net.org/download.php}{the ImageNet license}; others are not listed.}. We fine-tuned the models
on all these datasets for 50 epochs following~\cite{cai2020tinytl}. We also include VWW dataset~\cite{chowdhery2019visual}, a widely used benchmark for tinyML applications. We train on VWW for 10 epochs following~\cite{lin2020mcunet}. We used resolution 128 for all datasets and models for a fair comparison.

\myparagraph{Memory estimation.}
The memory usage of a computation graph is related to its implementation~\cite{ahn2020ordering, liberis2019neural, lin2020mcunet, lin2021mcunetv2}. We provide two settings for memory measurement: (1) \textbf{analytic profiling}: we count the size of \emph{extra} tensors required for backward computation, including the saved intermediate activation, binary truncation task, and the updated weights. The size is implementation-agnostic. It is used for a fast profiling;  (2) \textbf{on-device profiling}: we measure the actual memory usage when running model training on an STM32F746 MCU (320KB SRAM, 1MB Flash). We used TinyEngineV2~\cite{lin2021mcunetv2} as the backend and 2$\times$2 patch-based inference~\cite{lin2021mcunetv2} for the initial stage to reduce the forward peak memory. The \emph{measured} memory determines whether a solution can be deployed on the hardware.


\subsection{Experimental Results}
\label{sec:exp_qas}

\myparagraph{Quantization-aware scaling (QAS) addresses the optimization difficulty.}
We fine-tuned the last two blocks (simulate low-cost fine-tuning) of MCUNet to various downstream datasets (Table~\ref{tab:optimizer_study}). With momentum SGD, the training accuracy of the quantized model (\texttt{int8}) falls behind the floating-point counterpart due to the optimization difficulty.
Adaptive learning rate optimizers like Adam~\cite{kingma2014adam}  can improve the accuracy but are still lower than the \texttt{fp32} fine-tuning results; it also costs \textbf{3$\mathbf{\times}$ memory} consumption due to second-order momentum, which is not desired for tinyML settings. LARS~\cite{you2017large} cannot converge well on most datasets despite extensive hyper-parameter tuning (over both learning rate and the "trust coefficient"). We hypothesize that the aggressive gradient scaling rule of LARS makes the training unstable.
The accuracy gap is closed when we apply QAS, matching the accuracy of floating-point training at no extra memory cost.
We also provide the training curves of MCUNet on the Cars dataset w/ and w/o QAS in Figure~\ref{fig:training_curves_short}. QAS effectively helps optimization.

\input{mcunetv3/figure_text/tab_optimizer_study}

\begin{figure*}[t]
    \centering
     \includegraphics[width=0.85\textwidth]{mcunetv3/figures/training_curves_short.pdf}
    \caption{Training and validation loss curves w/ and w/o QAS. QAS effectively helps convergence, leading to better accuracy. The results are from updating the last two blocks of the MCUNet model on the Cars dataset.
    }
    \label{fig:training_curves_short}
\end{figure*}



\input{mcunetv3/figure_text/fig_acc_vs_mem}
\myparagraph{Sparse update obtains better accuracy at lower memory.}
We compare the performance of our searched sparse update schemes with two baseline methods: fine-tuning only biases of the last $k$ layers; fine-tuning weights and biases of the last $k$ layers. For each configuration, we measure the average accuracy on the 8 downstream datasets and the \emph{analytic} extra memory usage. We also compare with a simple baseline by only fine-tuning the classifier. As shown in Figure~\ref{fig:acc_vs_mem}, the accuracy of classifier-only update is low due to the limited learning capacity. \emph{Updating the classifier alone is not enough; we also need to update the backbone.} Bias-only update outperforms classifier-only update but the accuracy quickly plateaus and does not improve even more biases are tuned. For updating last $k$ layers, the accuracy generally goes higher as more layers are tuned; however, it has a very large memory footprint. Take MCUNet as an example, updating the last two blocks leads to an extra memory surpassing 256KB, making it infeasible for IoT devices/microcontrollers.
Our sparse update scheme can achieve higher downstream accuracy at a much lower memory cost: compared to updating last $k$ layers, sparse update can achieve higher downstream accuracy at \textbf{4.5-7.5$\times$} smaller memory overhead. 
We also measure the highest accuracy achievable by updating the last $k$ layers\footnote{Note that fine-tuning the entire model does not always lead to the best accuracy. We grid search for the best $k$ on Cars dataset: $k=$36 for MobileNetV2, 39 for ProxylessNAS, 12 for MCUNet, and apply it to all datasets.} as the baseline upper bound (denoted as "upper bound"). Interestingly, our sparse update achieves a better downstream accuracy compared to the baseline best statistics. We hypothesize that the sparse update scheme alleviates over-fitting or makes momentum-free optimization easier. 

\myparagraph{Matching cloud training accuracy for tinyML.} Remarkably, the downstream accuracy of our on-device training has \emph{matched or even surpassed} the accuracy of cloud-trained results on tinyML application VWW~\cite{chowdhery2019visual}. Our framework uses 206KB \emph{measured} SRAM while achieving 89.1\% top-1 accuracy for on-device training (we used gradient accumulation for the VWW dataset; see the appendix Section~\ref{sec:training_details} for details). The result is higher than the accuracy of the same model reported by the state-of-the-art solution MCUNet (88.7\%, trained on cloud and deployed to MCU). Both settings transfer the ImageNet pre-trained model to VWW. The on-device accuracy is far above the common requirement for tinyML (>80\% by MLPerf Tiny~\cite{banbury2020benchmarking}) and surpassed the results of industry solution TF-Lite Micro+MobileNetV2 (86.2\%~\cite{lin2020mcunet} under 256KB, \emph{inference-only, no  training support}).

\input{mcunetv3/figure_text/fig_latency_peakmem_comparison}
\myparagraph{\engine: memory saving.}
We measure the training memory of three models on STM32F746 MCU to compare the memory saving from \engineshort. We measure the peak SRAM usage under three settings: general full update, sparse update, and sparse update with TTE graph reordering (Figure~\ref{fig:latency_peakmem_comparison}(a)).
The sparse update effectively reduces peak memory by 7-10$\times$ compared to the full update thanks to the graph pruning mechanism, while achieving the same or higher transfer learning accuracy (compare the data points connected by arrows in Figure~\ref{fig:acc_vs_mem}). The memory is further reduced with operator reordering, leading to 22-28$\times$ total memory saving. With both techniques, the training of all 3 models fits 256KB SRAM.
We also compare the memory saving of reordering under different update schemes on MCUNet (Figure~\ref{fig:acc_vs_mem}(b), indicated by different accuracy levels).
Reordering consistently reduces the peak memory for different sparse update schemes of varying learning capacities.


\myparagraph{\engine: faster training.}
We further measure the training latency per image on the STM32F746 MCU with three settings: full update with TF-Lite Micro kernels, sparse update with TF-Lite Micro kernels, and sparse update with TTE kernels (Figure~\ref{fig:latency_peakmem_comparison}(c)). Notice that TF-Lite \emph{does not} support training; we just used the kernel implementation to measure latency.
By graph optimization and exploiting multiple compiler optimization approaches (such as loop unrolling and tiling), our sparse update + TTE kernels can significantly enhance the training speed by 21-23$\times$ compared to the full update + TF-Lite Micro kernels, leading to energy saving and making training practical. Note that TF-Lite with full update leads to OOM, so we report the projected latency according to the average speed of each op type (marked in dashed columns).


\subsection{Ablation Studies and Analysis}

\input{mcunetv3/figure_text/fig_visualize_scheme}
\myparagraph{Dissecting update schedules.}
We visualize the update schedule of the MCUNet~\cite{lin2020mcunet} model searched under 100KB extra memory (analytic) in Figure~\ref{fig:update_scheme} (lower subfigure (b), with 10 classes). It updates the biases of the last 22 layers, and sparsely updates the weights of 6 layers (some are sub-tensor update).
The initial 20 layers are frozen and run forward only. To understand why this scheme makes sense, we also plot the memory cost from activation and weight when updating \emph{each} layer in the upper subfigure (a). We see a clear pattern: the activation cost is high for the initial layers; the weight cost is high for the ending layers; while the total memory cost is low when we update the middle layers (layer index 18-30). The update scheme matches the memory pattern: to skip the initial stage of high activation memory, we only update biases of the later stage of the network; we update the weights of 4 intermediate layers due to low overall memory cost; we also update the partial weights of two later layers (1/8 and 1/4 weights) due to their high contribution to the downstream accuracy (Figure~\ref{fig:sensitivity_curve}). Interestingly, all the updated weights are from the first point-wise convolution in each inverted residual block~\cite{sandler2018mobilenetv2} as they generally have a higher contribution to accuracy (the peak points on the zigzag curve in Figure~\ref{fig:sensitivity_curve}(b)). 


\myparagraph{Effectiveness of contribution analysis.} We verify if the update scheme search based on contribution analysis is effective. We collect several data points during the search process (the update scheme and the search criteria, \ie, the sum of $\Delta\text{acc}$). We train the model with each update scheme to get the average accuracy on the downstream datasets (the real optimization target) and plot the comparison in Figure~\ref{fig:sensitivity_curve}(c). We observe a positive correlation, indicating the effectiveness of the search.





\myparagraph{Sub-channel selection.}
Similar to weight pruning, we need to select the subset of channels for sub-tensor update. 
We update the last two blocks of the MCUNet~\cite{lin2020mcunet} model and only 1/4 of the weights for each layer to compare the accuracy of different channel selection methods (larger magnitude, smaller magnitude, and random). The results are quite similar (within 0.2\% accuracy difference). Channel selection is not very important for transfer learning (unlike pruning). 
We choose to update the channels with a larger weight magnitude since it has slightly higher accuracy.



==> mcunetv3/text/5_conclusion.tex <==
\vspace{-5pt}
\section{Conclusion}
\label{sec:conclusion}
\vspace{-5pt}
In this paper, we propose the first solution to enable tiny on-device training on microcontrollers under a tight memory budget of 256KB. Our algorithm system co-design solution significantly reduces the training memory (more than 100$\times$ compared to existing work) and per-iteration latency, allowing us to obtain higher downstream accuracy. Our study suggests that tiny IoT devices can not only perform inference but also continuously adapt to new data for lifelong learning.

\myparagraph{Limitations and societal impacts.}
Our work achieves the first practical solution for transfer learning on tiny microcontrollers. However, our current study is limited to vision recognition with CNNs. In the future, we would like to extend to more modalities (\eg, audio) and more models (\eg, RNNs, Transformers). 
Our study improves tiny on-device learning, which helps to protect the privacy on sensitive data (\eg, healthcare). However, to design and benchmark our method, we experimented on many downstream datasets, leading to a fair amount of electricity consumption. 

\section*{Acknowledgments}
We thank National Science Foundation (NSF), MIT-IBM Watson AI Lab, MIT AI Hardware Program, Amazon, Intel, Qualcomm, Ford, Google for supporting this research.





==> text/5_tiny_federated.tex <==
\subsection{Federated TinyML}
\label{tiny_federated}
TinyML enables deep learning on a single embedded device. 
By combining TinyML with federated learning, it is possible to train local models on each device, and then use federated aggregation to collect the model updates and improve the global model. 
This can protect data privacy, as the data remains on the edge devices and is never transmitted to a central server (e.g., keyboard input history~\cite{google2016federated}, healthcare~\cite{rieke2020fl_healthcare}).
Studies have shown possible problems of data leakage from gradients~\cite{zhu2021dga}, which can be prevented by gradient pruning~\cite{lin2017deep}. The communication latency and bandwidth are another challenge of tiny federated learning, which can be solved by gradient compression~\cite{lin2017deep} and delayed gradient aggregation~\cite{zhu2021dga}.


%% ChatGPT
% TinyML enables deep learning on a single embedded device. By combining TinyML with federated learning, it is possible to train local models on each device and then use federated aggregation to collect model updates and improve the global model. This can protect data privacy, as the data remains on the edge devices and is never transmitted to a central server (e.g., keyboard input history~\cite{google2016federated}, healthcare~\cite{rieke2020fl_healthcare}). However, there are potential issues with data leakage from gradients~\cite{zhu2021dga}, which can be prevented through gradient pruning~\cite{lin2017deep}. Another challenge of tiny federated learning is communication latency and bandwidth, which can be addressed through gradient compression~\cite{lin2017deep} and delayed gradient aggregation~\cite{zhu2021dga}.


% \ligeng{TODO: related work and algos about federated learning.}
% \ligeng{TODO: add one more figure about federated learning.}
% \ligeng{What is federated TinyML? from single device to multiple devices}

% TinyML enables deep learning on embedded systems and typically use a small amount of data to run efficiently on \textit{single} devices. Naturally, people are interested in combining multiple devices as the IoT devices are ubiquitous in our daily life.  Federated learning, is a distributed machine learning approach that allows multiple devices to collaborate in training a machine learning model. In federated learning, each device trains a local model on its own data and then sends the model parameters to a central server, where they are aggregated and used to update a global model. This allows for the training of models using data from a large number of devices, without the need for that data to be centralized or shared among the devices.

% Federated learning can be useful in situations where data is distributed across multiple parties and cannot be easily shared, such as when working with sensitive data such as finical and medical records. This technique has been used to train models for medical treatments across multiple hospitals~\cite{jochems2016distributed}, analyze patient survival situations from various countries~\cite{jochems2017developing} and build predictive keyboards to improve typing experience~\cite{mcmahan2016communication, google2016federated, bonawitz2019towards}.

% TinyML and federated learning can be used together to enable machine learning on a group of tiny devices. For example, a federated learning system could use TinyML algorithms to train local models on each device, and then use federated learning techniques to aggregate the model updates and improve the global model. In this way, TinyML and federated learning can enable efficient and privacy-preserving machine learning on a large number of devices.

% \subsection{DGA: enable federated learning under high latency}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/fig1_settings-crop.pdf}
%     \caption{\textit{Left}, \textit{Middle}: The training settings of conventional distributed training v.s. federated learning are very different. \textit{Right}:  High latency cost greatly degrades the FedAvg's~\cite{mcmahan2016communication} performance, proposing a severe challenge to scale up the training system. The latency statistics is referenced from Verizon~\cite{verizon_latency} and speedtest~\cite{speedtest_latency}.
%     }
%     \label{fig:settings}
%     % \vspace{-0.5cm}
% \end{figure*}

% While the bandwidth constraints have been efficiently addressed by gradient compression~\cite{lin2017deep}, low-rank updates~\cite{google2016federated} and quantization techniques~\cite{sun2019optimizing}, the issue related to network latency is rarely studied in the recent literature~\cite{kairouz2019advances, hsieh2017gaia}. However, high network latency is inevitable in federated settings because of (1) wireless connections and (2) long-distance transmission (Figure.~\ref{fig:settings}.(b)). On the one hand, the high-density urban office and home environments create a lot of contention, as dozens of devices compete for the same radio frequency. On the other hand, the multi-geographic located data entails a minimum latency cost: even with the speed of light, it requires hundreds of milliseconds to send a packet across the world. In either case, the high latency is a hard barrier introduced by physical limits thus inevitable. If not handled specifically, such communication lag, in the magnitude of hundreds of milliseconds, or even seconds, will significantly degrade the scalability of the learning algorithm as shown in the Figure.~\ref{fig:settings}.

% We propose \textbf{D}elayed \textbf{G}radient \textbf{A}ggregation () to address the latency bottleneck. The key idea is to delay the gradient averaging to a future iteration thus the communication can be pipelined with computation. By accepting stale average gradients for model updates, DGA allows the communication to execute in parallel with the computation, thus scalable even under extreme latency. 
% % We prove that our DGA shares the same convergence as FedAvg and provide extensive experiments on image and language tasks in both i.i.d. and non-i.i.d settings. We demonstrate that (i) DGA speeds up FedAvg by a factor 2.6$\times$ to 4.1$\times$ over various datasets; (ii) no accuracy drop under extreme communication lag (e.g., > 1 second). We further set up a Raspberry Pi cluster to simulate the real-world scenario and demonstrate that DGA is robust against network stragglers. 

% \begin{figure*}
%     \centering
%     % \includegraphics[width=\linewidth]{figures/fig_method-crop.pdf}
%     \begin{subfigure}{0.8\linewidth}
%         \includegraphics[width=\linewidth]{figures/fig_method_fedavg-crop.pdf}
%         \caption{Federated Averaging: $K$ indicates how many local steps before the averaging starts.}
%         \label{fig:method:fedavg}
%     \end{subfigure}
%     % \begin{subfigure}{0.8\linewidth}
%     %     \includegraphics[width=\linewidth]{figures/fig_method_dga-crop.pdf}
%     %     \caption{Delayed Gradient Averaging: $D$ indicates how many delayed steps before the averaging finishes.}
%     %     \label{fig:method:dga}
%     % \end{subfigure}
%     \caption{\ligeng{Remake the figures to shrink height}. We provide another interpretation of our algorithm, iterating over the gradient iterations, for instance, the $(tK+k)$-th iteration in the pseudo code represents the $t$-th round $k$-th iterations in Algorithm~\ref{algo}. The averaging occurs periodically with period $K$ and the delay parameter $D$ naturally shows up indicating the number of gradients between the sending and reception. The cyan cube in the visualization (a,b) indicates local computation and the yellow cube represents the transmission of the averages. The red bar indicates when the averaging is actually performed. In, the transmission is in parallel to the computation, which is the main reason why ~can tolerate high latency.}
%     \label{fig:method}
% \end{figure*}

% The main idea of our algorithm is to allow local updates during the communication of the averaging. In FedAvg, clients send its parameter to each other at the end of each round, wait until the averaging (communication) ended, later starts the next round. In our algorithm, \textbf{the averaging barrier is delayed to a later iteration} so that clients can immediately start the next round and \textbf{an gradient correction term is designed to compensate the staleness}:

% % \begin{enumerate}[leftmargin = 0.2in]
% %     \item Clients send updates to each other at the end of $t$-th round;
% %     \item Clients continue performing local updates using the latest local parameter; 
% %     \item When other's $t$-th round info arrived, the client has already performed $D$ extra local updates.
% %     \item Delayed averaging step: replace the local gradients at the $t$-th round by the received averaging (we will detail this step right away).  
% % \end{enumerate}

% The benefit is plain to see: we no longer freeze the local computation power during the communication. 
% % Now, the difficulty lies in the additional staleness coming with the delayed averaging. 
% % To make the discussion more explicit, we denote the parameter on the $i$-th client at the $k$-th iteration within the $t$-th round by $w^i_{t,k}$ and the corresponding stochastic gradient as $g^i_{t,k}$. In the very first round $t=1$, solely local updates are performed, hence the last iterate in the first round can be expressed as
% % % \vspace{-0.2cm}
% % \[  w_{1,K+1}^i =  w_{1,K}^i - \eta g_{1,K}^i = \cdots =  w_{1} - \eta \underbrace{\color{purple}{\sum_{k=1}^K g_{1,k}^i}}_{:= m_1^i }. \]

% \begin{wrapfigure}{r}{0.25\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/pi_cluster.png}
%     \caption{Our Raspberry Pi farm. Experiments are conducted on two racks.}
%     \vspace{-0.8cm}
%     \label{fig:pi_cluster}
% \end{wrapfigure}


% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.4\linewidth]{figures/pi_cluster.png}
% %     \caption{Our Raspberry Pi farm. Experiments are conducted on two racks.}
% %     \label{fig:pi_cluster}
% % \end{figure}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/scale_across-crop.pdf}
%     \label{fig:scale_rapsberry_pi}
%     \caption{The speedup comparison between FedAvg and on Raspberry Pi cluster. On both vision and language tasks, \ours~demonstrate consistent improvement over FedAvg. \ligeng{merge with Pi figures}}
%     \label{exp:pi_scalability}
%     % \vspace{-15pt}
% \end{figure*}

% we benchmark real-world settings on the Raspberry Pi cluster in the Figure.~\ref{exp:latency_vs_throughput:synthetic}.. 
% Instead of simulating different latency settings, we consider four representative cases for federated learning 
% [i] wired [ii] (wireless) different rooms [iii] (wireless) different floors [iv] (wireless) different buildings, where the latency numbers are 1ms, 16ms and 132ms and 470ms respectively.  
% By placing the Pi cluster at different locations, we can emulate different quality of connection. Different from synthetic latency, the real wireless connection also suffers from unpredictable network stragglers and packet loss, thus the overall throughput on Pi-clusters is worse and FedAvg's performance degrades more quickly.
% Even under such challenging network, the throughput of DGA remains steady.

% Figure.~\ref{exp:pi_scalability} shows the speedup ratio (scalability) on the Pi cluster. 
% We adopt small models LeNet and 2-layer lstm for the benchmark. Given the limited computation budget of edge devices, the batch size is reduced to 1/8 of the original ones. 
% To better evaluate our algorithm, we choose the most challenging settings where devices are linked through wireless connections from different buildings. 
% With an average latency of 470ms, FedAvg's training is significantly slowed by the communication. When scaling the training to two devices, the speedup ratio is only 0.6, which is even slower than single devices. 
% Instead, our proposed DGA demonstrates ideal scalability under a high-latency network. When scaling to eight devices, the speedup ratio is about 13.1. This performance is close to what conventional algorithms achieved inside a data center.

% \subsection{Potential Leakages from Gradients}
% % write the half page to explain the setup and potential impacts
% \ligeng{}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/fig2-crop.pdf}
%     \caption{The overview of our DLG algorithm. Variables to be updated are marked with a bold border. While normal participants calculate $\nabla W$ to update parameter using its private training data, the malicious attacker updates its dummy inputs and labels to minimize the gradients distance. When the optimization finishes, the evil user is able to steal the training data from honest participants.
%     }
%     \label{fig:methods}
% \end{figure}

% % \input{figure_text/dlg_algorithm.tex}

% Collaborative learning have been widely used in large scale machine learning tasks. However, \textbf{does the ``gradient sharing'' scheme protect the privacy of the training datasets of each participant?} 
% In most scenarios, people assume that gradients are safe to share and will not expose the training data. Some recent studies show that gradients reveal some properties of the training data, for example, property classifier~\cite{Melis2018unintended} (whether a sample with certain property is in the batch) and using generative adversarial networks to generate pictures that look similar to the training images~\cite{hitaj2017information, Melis2018unintended, fredrikson2015model_inversion}. 
% Here we consider a more challenging case: can we \textbf{completely} steal the training data from gradients? 
% Formally, given a machine learning model $F()$ and its weights $W$, if we have the gradients $\nabla w$ w.r.t a pair of input and label, can we obtain the training data reversely? 


% Conventional wisdom suggests that the answer is no. Previous ``shallow'' leakages (property inference~\cite{shokri2017membership, Melis2018unintended} and generative model~\cite{hitaj2017information} using class labels) requires extra label information and can only generate similar synthetic images.  But recent work \emph{Deep Leakage from Gradients} (\textbf{DLG})~\cite{zhu2019dlg} reveals that sharing the gradients can leak private training data. \textbf{DLG} presents an optimization algorithm that can obtain both the training inputs and the labels in just few iterations.  Specifically, consider standard synchronous distributed training: At each step $t$,  every node $i$ samples a minibatch 
% % $(\mathbf{x}_t, \mathbf{y}_t) =  \{ x_{t, j}, y_{t, j} \} _{j=1}^{n} $ 
% $(\mathbf{x}_{t, i}, \mathbf{y}_{t, i}) $
% from its own dataset to compute the gradients


% \input{figures/experiments/vision.tex}

% The leaking process is visualized in Fig.~\ref{fig:experiment_vision}. We start with random Gaussian noise (first column) and try to match the gradients produced by the dummy data and real ones. As shown in Fig~\ref{fig:vision_fig3}, minimizing the distance between gradients also reduces the gap between data. We observe that monochrome images with a clean background (MNIST) are easiest to recover, while complex images like face take more iterations to recover (Fig.~\ref{fig:experiment_vision}). When the optimization finishes, the recover results are almost identical to ground truth images, despite few negligible artifact pixels.

% We visually compare the results from other method~\cite{Melis2018unintended} and ours in Fig.~\ref{fig:experiment_vision}. 
% The previous method uses GAN models when the class label is given and only works well on MNIST. The result on SVHN, though is still visually recognizable as digit ``9'',  is no longer the original training image. The cases are even worse on LFW and totally collapse on CIFAR. We also make a numerical comparison by performing leaking and measuring the MSE on all dataset images in Fig.~\ref{fig:vision_fig_bar}. Images are normalized to the range $[0, 1]$ and our algorithm appears much better results (ours $< 0.03$ v.s. previous $> 0.2$) on all four datasets.

% \begin{figure*}[t]
%     \centering
%     % \includegraphics[width=\linewidth]{figures/fig4}
%     % \caption{Caption \SH{font size should be as large as main text; reduce the space between the two rows}}
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/fig5_gaussian-crop.pdf}
%         \caption{Defend with different magnitude Gaussian noise.}
%         \label{fig:defense:gaussian}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.49\textwidth}
%     %     \centering
%     %     \includegraphics[width=\textwidth]{figures/fig5_laplacian-crop.pdf}
%     %     \caption{Defend with different magnitude Laplacian noise.}
%     %     \label{fig:defense:Laplacian}
%     % \end{subfigure} 
%     % \\ \vspace{4pt}
%     % \begin{subfigure}[b]{0.49\textwidth}
%     %     \centering
%     %     \includegraphics[width=\textwidth]{figures/fig5_fp16-crop.pdf}
%     %     \caption{Defend with fp16 convertion.}
%     %     \label{fig:defense:fp16}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/fig5_dgc-crop.pdf}
%         \caption{Defend with gradient pruning.}
%         \label{fig:defense:dgc}
%     \end{subfigure} 
%     \caption{The effectiveness of various defense strategies. }
%     \label{fig:defense}
%     \vspace{-5pt}
% \end{figure*}


% \subsection{Defense }

% One straightforward attempt to defense DLG is to add noise on gradients before sharing. 
% % 
% % This action has been empirically proved that only has little effects on performance, however, will make the DLG side optimization difficult.  
% % 
% To evaluate, we experiment  Gaussian and Laplacian noise (widely used in differential privacy studies) distributions with variance range from $10^{-1}$ to $10^{-4}$ and central $0$. From Fig.~\ref{fig:defense:gaussian} and \ref{fig:defense:Laplacian}, we observe that the defense effect mainly depends on the magnitude of distribution variance and less related to the noise types. When variance is at the scale of $10^{-4}$, the noisy gradients do not prevent the leak. For noise with variance $10^{-3}$, though with artifacts, the leakage can still be performed. Only when the variance is larger than $10^{-2}$ and the noise is starting to affect the accuracy, DLG will fail to execute and Laplacian tends to slight better at scale $10^{-3}$. However, noise with variance larger than $10^{-2}$ will degrade the accuracy significantly (Tab.~\ref{tab:defense_vs_accuracy}).

% Another common perturbation on gradients is half-precision, which was initially designed to save GPU memory footprints and also widely used to reduce communication bandwidth. We test two popular half-precision implementations IEEE float16 (\textit{Single-precision floating-point format}) and bfloat16 (\textit{Brain Floating Point}~\cite{tagliavini2017transprecision}, a truncated version of 32 bit float). Shown in Fig.~\ref{fig:defense:fp16},  both half-precision formats fail to protect the training data. We also test another popular low-bit representation Int-8. Though it successfully prevents leakage, the performance drops seriously (Tab.~\ref{tab:defense_vs_accuracy}).


% \subsubsection{Gradient Compression and Sparsification} \label{sec:defense:few_gradients}
% % Beside perturbing the gradients, another defense approach is to sparsify the gradients~\cite{DGC}, an effective  
% We next experimented to defend by gradient compression~\cite{lin2017deep, tsuzuku2018variance}: Gradients with small magnitudes are pruned to zero. It's more difficult for DLG to match the gradients as the optimization targets are pruned.
% % 
% We evaluate how different levels of sparsities (range from 1\% to 70\%) defense the leakage. When sparsity is 1\% to 10\%, it has almost no effects against DLG. When prune ratio increases to 20\%, as shown in Fig.~\ref{fig:defense:dgc}, there are obvious artifact pixels on the recover images.  
% % 
% We notice that the maximum tolerance of sparsity is around 20\%. 
% When pruning ratio is larger, the recovered images are no longer visually recognizable and thus gradient compression successfully prevents the leakage.

% Previous work~\cite{tsuzuku2018variance, lin2017deep} show that gradients can be compressed by more than 300$\textbf{}\times$ without losing accuracy by error compensation techniques. In this case, the sparsity is above 99\% and already exceeds the maximum tolerance of DLG (which is around 20\%). It suggests that compressing the gradients is a practical approach to avoid the deep leakage. 



% % TinyML: MCU scope, 
% % broader design: IoT
% % more broader: efficient, scalable
